Training and Evaluation of Deep Policies using Reinforcement Learning and Generative Models

We present a data-efficient framework for solving sequential decision-making problems which exploits the combination of reinforcement learning (RL) and latent variable generative models. The framework, called GenRL, trains deep policies by introducing an action latent variable such that the feed-forward policy search can be divided into two parts: (i) training a sub-policy that outputs a distribution over the action latent variable given a state of the system, and (ii) unsupervised training of a generative model that outputs a sequence of motor actions conditioned on the latent action variable. GenRL enables safe exploration and alleviates the data-inefficiency problem as it exploits prior knowledge about valid sequences of motor actions. Moreover, we provide a set of measures for evaluation of generative models such that we are able to predict the performance of the RL policy training prior to the actual training on a physical robot. We experimentally determine the characteristics of generative models that have most influence on the performance of the final policy training on two robotics tasks: shooting a hockey puck and throwing a basketball. Furthermore, we empirically demonstrate that GenRL is the only method which can safely and efficiently solve the robotics tasks compared to two state-of-the-art RL methods.

==> original/inputs/abstract.tex <==
\begin{abstract}
We present a data-efficient framework for solving visuomotor sequential decision-making problems which exploits the combination of reinforcement learning (RL) and latent variable generative models. Our framework trains deep visuomotor policies by introducing an action latent variable such that the feed-forward policy search can be divided into three parts: (i) training a sub-policy that outputs a distribution over the action latent variable given a state of the system, (ii) unsupervised training of a generative model that outputs a sequence of motor actions conditioned on the latent action variable, and (iii) supervised training of the deep visuomotor policy in an end-to-end fashion. Our approach enables safe exploration and alleviates the data-inefficiency problem as it exploits prior knowledge about valid sequences of motor actions. Moreover, we provide a set of measures for evaluation of generative models such that we are able to predict the performance of the RL policy training prior to the actual training on a physical robot. We define two novel measures of disentanglement and local linearity for assessing the quality of latent representations, and complement them with existing measures for assessment of the learned distribution. We experimentally determine the characteristics of different generative models that have the most influence on performance of the final policy training on a robotic picking task.
%Moreover, by evaluating the quality of the generative models we are able to predict the performance of the RL policy training prior to the actual training on a physical robot. We achieve this by defining two novel measures of disentanglement and local linearity for assessing the quality of generative models' latent spaces, and complementing them with the existing measures for evaluation of generative models. We demonstrate the efficiency of our approach on a robotic picking task using several different generative models and determine which of their properties have the most influence on performance of the final policy training.   
\end{abstract}

==> original/inputs/algorithm.tex <==
\begin{algorithm}[h]
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\caption{Pseudocode of the EM policy training based on generative models.}
\Input{generative model $g_\vartheta$, initial policy $\pi_\theta$, initial value function $V_\pi$, batch size $N$}
\Output{trained $\pi_\theta$}
\While{training $\pi_\theta$}{
\For{$i = 1, \dots, N$}{
sample states $s_i \sim p(s)$ \\
sample actions $\alpha_i \sim \pi_\theta(.|s_i)$ \\
generate motor actions $\tau_i \leftarrow g_\vartheta(\alpha_i)$  \\
obtain the rewards $r_i\leftarrow r(s_i, \tau_i)$ \\
}
\Repeat{training done}{
\textbf{E-step:} \\
\quad update the variational policy $q_\phi$ according to~\eqref{eq:trpo} given $\{s_i, \alpha_i, r_i\}_{i=1}^N$ \\
\textbf{M-step:} \\
\quad update the policy $\pi_\theta$ according to~\eqref{eq:M_loss} given $q_\phi$ and $\{s_i, \alpha_i\}_{i=1}^N$\\
}
update the value function $V_\pi$ given $\{s_i,r_i\}_{i=1}^N$\\
}
\label{alg:training}
\end{algorithm}


==> original/inputs/background.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

\begin{figure}[ht]
\centering
\includegraphics[width=0.7\linewidth]{figures/policy_network_img_cropped.pdf} 
\caption{The architecture of the deep action-selection policy $\pi_\Theta$ based on latent-variable generative models. The policy consists of two models, the sub-policy $\pi_\theta(\alpha|s')$ that assigns a distribution over the action latent variable $\alpha$ conditioned on a given state $s'$, and a generative model $\tau' = g_\vartheta(\alpha')$ that maps a latent action sample $\alpha' \sim \pi_\theta(\alpha|s')$  into a trajectory of motor actions $\tau'$. Given the initial state $s'$ and the action trajectory $\tau'$ that is executed on the robot, the environment returns a terminal reward $r'$ according to the reward probability $r' \sim p(r|s',\tau')$.}\label{fig:deep_policy_network}
\end{figure}

We consider a finite-horizon Markov decision process defined by a tuple $(\mathbf{S}, \mathbf{U}, P, p(s), p(r|s,\tau))$ where $\mathbf{S} = \mathbb{R}^{N_s}$ is a set of $N_s$-dimensional states, $\mathbf{U}$ is a set of motor actions $u_{m}$ for the robot motor $m$, %at the time index $t$, 
$P: \mathbf{S} \times \mathbf{U} \times \mathbf{S} \rightarrow \mathbb{R}$ is the state transition probability, and $p(s)$ is the initial state distribution. The probability $p(r|s',\tau')$ of the reward $r$, conditioned on a state $s'$ and a fixed-length sequence $\tau' = (u_{t, m})$ of motor $m$ actions $u_{t, m}$ at time step $t$, is unknown to the learning agent.
%a fixed number of motor actions $\tau' = \{u_{ m}\}$, is unknown to the learning agent.
%Our framework consists of three parts: (1) policy training using EM algorithm combined with generative models, (2) training and evaluation of the generative models, and (3) training of the perception module. In this section, we introduce the problem of training a feed-forward deep policy network and describe our approach to solving it by leveraging generative models. We then present each of the three parts of the framework in the following section.
%We deal with episodic tasks where the goal is to find a sequence of actions $\tau' = \{a_{t,m}\} \in \mathbb{R}^{T\times M}$ consisting of $T$ time-steps and $M$ motor actions for a given state $s' \in \mathbb{R}^{N_s}$. More specifically, 
We wish to find a policy $\pi_\Theta(\tau|s')$ %represented by a deep neural network $\Theta$, 
based on which a sequence of motor actions $\tau'$ can be sampled given a state of the environment $s'$.
The state contains information about the current configuration of the environment as well as the goal to reach in case a goal-conditioned policy has to be obtained. 
%For a given state $s'$ and a sequence of actions $\tau'$ a reward $r$ is given at the end of each trial according to the reward probability distribution $p(r| s', \tau')$ which is unknown to the learning agent.
%The problem is to find a deep policy $\pi_\theta(\tau|s)$ based on which a sequence of motor actions $\tau$ can be sampled conditioned on the state of the task $s$. 
%The policy parameters have to be obtained such that the likelihood of receiving high rewards is maximized. 
Let $r^*$ be the minimum reward required to successfully complete the task.
The policy $\pi_\Theta$ is represented by a neural network with parameters $\Theta$ that are trained to maximize the probability of receiving high rewards $p(r \ge r^*|s', \tau')$ % by marginalizing over all trajectories
\begin{equation}
\begin{split}
    \Theta^* & = \argmax_{\Theta} \iint p(s)\, \pi_{\Theta}(\tau | s)\, p(r|s,\tau)\, ds \, d\tau \\
     & = \argmax_{\Theta} \mathbb{E}_{s' \sim p(s), \tau' \sim \pi_{\Theta}(\tau|s')} [\, p(r | s', \tau')\,],
    \label{eq:margin_tau}
\end{split}
\end{equation}
%where $p(s)$ denotes the initial distribution over states. 
where we omitted the reward threshold $r^*$ for simplicity.
Our approach is based on training a generative model $g_\vartheta$, parametrized by $\vartheta$, that maps a low-dimensional latent action sample $\alpha' \in \mathbb{R}^{N_\alpha}$ into a motion trajectory $\tau' \in \mathbb{R}^{T\times M}$, where $N_\alpha \ll T\times M$. 
In other words, we assume that the search space is limited to the trajectories spanned by the generative model. 
In this case, the feed-forward policy search problem splits into two sub-problems: (i) finding the mapping $g_\vartheta(\alpha')$ and (ii) finding the sub-policy $\pi_\theta (\alpha | s')$, where $\Theta = [\theta, \vartheta]$. 
Instead of marginalizing over trajectories as in~\eqref{eq:margin_tau} we marginalize over the latent variable by exploiting the generative model
\begin{equation}
\theta^* = \argmax_{\theta} \mathbb{E}_{s' \sim p(s), \alpha' \sim \pi_{\theta}(\alpha|s')} [\, p(r|s', g_\vartheta(\alpha')\,)\,].
\label{eq:margin_alpha}
\end{equation}
An overview of our approach is shown in Figure~\ref{fig:deep_policy_network}. Once the models are trained the output of the policy $\pi_\Theta$ is found by first sampling from the sub-policy $\alpha' \sim \pi_\theta(\alpha | s')$ given a state $s'$ and then using the mapping $g_\vartheta$ to get the sequence of motor actions $\tau' = g_\vartheta(\alpha')$. The state $s'$ and the generated trajectory $\tau'$ are then given to the environment which outputs a reward $r'$.
In the rest of the text we refer to the sub-policy as the \textit{policy} and omit the parameters $\vartheta$ from the notation $g_\vartheta$ when they are not needed.
By abuse of notation, we will drop the explicit distinction between a random variable, e.g., $\alpha$, and a concrete instance of it, $\alpha'$, in the rest of the paper and only write $\alpha$ when no confusions can arise. %for the sake of simplicity. 
%There are four advantages to perform the policy search in the low-dimensional latent space:
%(1) the search space is considerably smaller compared to the high-dimensional trajectory space,
%(2) the sequential decision making problem is reduced to a contextual multi-armed bandit without temporal complexities and credit assignment problem, 
%(3) the exploration is done based on trajectories generated by the generative model which increases the safety of real robot explorations, and
%(4) it provides a natural way to exploit prior knowledge based on human demonstration or general trajectory planning algorithms. %this formulation provides a natural way to exploit prior knowledge for improving the efficiency of the learning process. 
In the following section, we introduce the expectation-maximization (EM) algorithm for training an action-selection policy using a generative model based on which different motor trajectories suitable for solving a given task can be generated. %We shortly describe VAEs and GANs and review which characteristics they need to possess to achieve an efficient policy training. 


==> original/inputs/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We presented an RL framework that combined with generative models trains deep visuomotor policies in a data-efficient manner. The generative models are integrated with the RL optimization by introducing a latent variable $\alpha$ that is a low-dimensional representation of motor actions. Using the latent action variable $\alpha$, we divided the optimization of the parameters $\Theta$ of the deep visuomotor policy $\pi_\Theta(\tau|s)$
into two parts: optimizing the parameters $\vartheta$ of a generative model $p_\vartheta(\tau|\alpha)$ that generates valid sequences of motor actions, and optimizing the parameters $\theta$ of a sub-policy $\pi_\theta(\alpha | s)$, where $\Theta = [\theta, \vartheta]$. The sub-policy parameters $\theta$ are found using the EM algorithm, while generative model parameters $\vartheta$ are trained unsupervised to optimize the objective corresponding to the chosen generative model. In summary, the complete framework consists of three data-efficient downstream tasks: 
(a) training the generative model $p_\vartheta$, (b) training the sub-policy $\pi_\theta$, and (c) supervised end-to-end training the deep visuomotor policy $\pi_\Theta$.

Moreover, we provided a set of measures for evaluating the quality of the generative models regulated by the RL policy search algorithms such that we can predict the performance of the deep policy training $\pi_\Theta$ prior to the actual training. In particular, we defined two new measures,  disentangling precision and recall ($\Dip$ and $\Dir$) and latent local linearity (L3), that evaluate the quality of the latent space of the generative model $p_\vartheta$, and complemented them with precision and recall measure \cite{kynkaanniemi2019improved} which evaluates the quality of the generated samples. We experimentally demonstrated the predictive power of these measures on a picking task using a set of different VAE and GAN generative models. %In case of GANs, we identify the disentangling recall $\Dir$ as well as local linearity
Regardless of the model type, we observe recall to be the most influential property, followed by precision in case of VAEs and by disentangling recall in case of GANs. 



==> original/inputs/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

In this section, we experimentally determine the characteristics of generative models that contribute to a more data-efficient policy training for a picking task performed on a real robotic platform. We first trained several $\beta$-VAE and InfoGAN models with various hyperparameters, and evaluated them by measuring disentanglement, local linearity as well as precision and recall introduced in Section~\ref{sec:eval_generative_model}. Using these models and the proposed EM algorithm presented in Section~\ref{sec:em_policy_training}, we then trained several RL policies and investigated the relation between the properties of the generative models and the performance of the policy.

Note that the experimental section of this work focuses solely on the evaluation of the generative models. Readers interested in the investigation of the data-efficiency of the proposed approach in training complex visuomotor skills are referred to \cite{ghadirzadeh2017deep}. Moreover, we emphasize that it is not meaningful to directly compare our approach to neither PPO nor GPS. Training a policy using PPO requires vast amounts of data, while GPS requires a reward at every time step instead of the terminal reward as in our case.

%We first trained deep visuomotor policy with the proposed EM algorithm presented in Section~\ref{sec:em_policy_training} for a picking task on a real robotic platform. In this case, the visuomotor policy maps raw image pixel values to a complete sequence of motor actions to pick an object at different positions and orientations on a tabletop.   

%We experimentally evaluated our proposed approach by training a deep visuomotor policy for a picking task on a real robotic platform. In this case, the visuomotor policy maps raw image pixel values to a complete sequence of motor actions to pick an object at different positions and orientations on a tabletop. We demonstrate that by dividing the training into three more manageable parts, the policy can be trained after a few hundred trials that can be safely executed on a physical robot.% in less than 30 minutes. 

%We then trained several $\beta$-VAE and InfoGAN models with various hyperparameters, and evaluated them by measuring disentanglement, local linearity as well as precision and recall introduced in Section~\ref{sec:eval_generative_model}. Using these models and the proposed EM algorithm, we trained several RL policies and investigated the relation between the properties of the generative models and the performance of the policy. 

%Finally, we investigated how the number of the variational policies affects the performance of the policy training by modifying the E-step of the EM algorithm. We chose a generative model that performed well in the single policy training task and evaluated the performance of the final policy training when deploying several variational policies. As the result, we can give the optimal number of variational policies that result in the best final policy training performance. 




 




%In this section, we present our experimental results aimed at answering the following questions:
%\begin{enumerate}
%    \item How does the proposed approach that divides the visuomotor policy training into several more manageable downstream tasks perform for end-to-end training of visuomotor policies?
%    \item Which of the characteristics precision and recall, disentanglement and local linearity of a generative model affect the policy training the most? 
%    \item How does the number of variational policies affect the performance of the policy training? What is the optimal number of the variational policies to speed up the training? 
%\end{enumerate}

%We answer (1) by training a deep visuomotor policy for a picking task on a real robotic platform. We demonstrate that a deep visuomotor policy can be be trained after a few hundreds of trials that can be safely executed on a physical robot in less than 30 minutes. In this case, the visuomotor policy maps raw image pixel values to a complete sequence of motor actions to pick an object at different positions and orientations on a tabletop. 

%%%%%By providing the results from our earlier study \cite{chen2019adversarial}, we motivate the use of the introduced adversarial domain adaptation algorithm to improve the generality of the obtained deep visuomotor policy. The policy is  general in the sense that it can manipulate novel task objects in a cluttered environment, a situation that has never been encountered during the policy training phase. 
%We emphasize that our approach cannot be directly compared to neither PPO nor GPS. Training a policy using PPO requires vast amounts of data, while GPS requires a reward at every time step instead of the terminal reward as in our case.

%We answer (2) by training several $\beta$-VAE and InfoGAN generative models with various hyperparameters and evaluate them using the measures introduced in Section~\ref{sec:eval_generative_model}. For each model, we train several RL policies based on the proposed EM algorithm and investigate how the performance is related to the discussed properties of the generative models.  

%Finally, we answer (3) by modifying the E-step of the EM algorithm to optimize for different number of variational policies. We choose a generative model that performed well in the single policy training task and evaluate the performance of the final policy training when deploying several variational policies. As the result, we can give the optimal number of variational policies that result in the best final policy training performance. 

\subsection{Experimental setup}
\label{sec:exp:setup}
We applied our framework to a picking task in which a 7 degree-of-freedom robotic arm (ABB YuMi) must move its end-effector to different positions and orientations on a tabletop to pick a randomly placed object on a table. In this case, raw image pixel value are given as the input to the visuomotor policy. This task is a suitable benchmark to answer our research questions. 
First of all, the task requires feed-forward control of the arm over 79 time-steps to precisely reach a target position without any position feedback during the execution.
Therefore, precision is an important factor for this problem setup. 
Secondly, reaching a wide range of positions and orientations on the tabletop requires the generative model $g$ to generate all possible combinations of motor commands that bring the end-effector to every possible target position and orientation. This means that $g$ needs to have a high recall. Thirdly, it is straightforward to evaluate the disentanglement of the latent representations  as well as the local linearity of the dynamical system that is formed by $g$ and the robot kinematic model. 
%A disentangled representation of the action sequences results in a new dynamical system in which every dimension of the state space, i.e., the space of the position and the orientation of the end-effector at the last time-step of the action sequence, is controllable by only one  dimension of the new action space, i.e., the latent action space of the generative model. The same argument can be made for the linearity of the resulting dynamical system. 
Finally, this is a suitable task for end-to-end training, especially by exploiting the adversarial domain adaptation technique in \cite{chen2019adversarial} to obtain generality for the policy training task. 
Note that the applicability of our framework (up to minor differences) to a wide range of robotic problems has already been addressed by our prior work. In particular, we successfully evaluated it in several robotic task domains, e.g., ball throwing to visual targets \cite{ghadirzadeh2017deep}, shooting hockey pucks using a hockey stick \cite{arndt2019meta}, pouring into different mugs \cite{hamalainen2019affordance}, picking objects \cite{chen2019adversarial}, and imitating human greeting gestures \cite{butepage2019imitating}. 

We constructed a dataset containing sequences of motor actions using MoveIt planners \cite{coleman2014reducing}.  
We collected $15750$ joint velocity trajectories to move the end-effector of the robot from a home position to different positions and orientations on a tabletop. 
The trajectories were sampled at $10$Hz and trimmed to 79 time-steps ($7.8$ seconds duration) by adding zeros at the end of the joint velocities that are shorter than 79 time-steps. 
The target positions as well as orientations consisting of Euler angles form a $N_s = 6$ dimensional end state space, and were sampled uniformly to cover an area of $750$ cm$^2 \times 3.1$ rad. 
%Furthermore, in our recent work, we have successfully evaluated the current framework (with minor differences) to solve sequential decision-making problems in several robotic task domains, e.g., ball throwing to visual targets \cite{ghadirzadeh2017deep}, shooting hockey pucks using a hockey stick \cite{arndt2019meta}, pouring into different mugs \cite{hamalainen2019affordance}, picking objects \cite{chen2019adversarial}, and imitating human greeting gestures \cite{butepage2019imitating}. 
%Therefore, the applicability of the solution for a wide range of robotic problems is already addressed by our prior work. 

\subsection{Generative model training}
\label{sec:exp:generative_model}
The generative models are represented by neural networks that map a low-dimensional action latent variable $\alpha$ into a $7\times79$ dimensional vector representing $7$ motor actions and $79$ time-steps. In total, we trained $9$ $\beta$-VAE models and $9$ InfoGAN models with latent dimension chosen from $N_\alpha \in \{2, 3, 6\}$.
We refer the reader to the Appendix \ref{app:gen_models} for the exact architecture of the models as well as all the training details. The prior distribution $p(\alpha)$ is the standard normal distribution $\text{N}(0, 1)$ in case of $\beta$-VAEs, and the uniform distribution $\text{U}(-1, 1)$ in case of InfoGANs. 

%The input size of the networks is the same as the dimension of the latent space $N_\alpha$. 
Table~\ref{tabel:exp:vae} summarizes the parameters of the $\beta$-VAE models together with the values of both the KL divergence and reconstruction term (right and left term in~\eqref{eq:vae}, respectively) obtained at the last epoch.
%The VAEs were trained with different $\beta$ parameters and latent sizes $N_\alpha \in \{2, 3, 6\}$. The parameters of each model together with the values of both the KL divergence term and the reconstruction term (right and left term in~\eqref{eq:vae}, respectively) are summarised in Table \ref{tabel:exp:vae}. 
At the beginning of training, we set $\beta = 0$ and gradually increase its value until the value of the KL divergence drops below a predetermined threshold 
set to $1.5, 2.5$ and $3.5$. The resulting $\beta$ value is reported in Table \ref{tabel:exp:vae} and kept fixed until the end of the training. 
Table \ref{tabel:exp:gan} summarizes the training parameters and loss function values of the InfoGAN models. We report the total model loss~\eqref{eq:gan} (M-loss), the generator loss (G-loss, middle term in~\eqref{eq:gan}) and the mutual information loss (I-loss, right term in~\eqref{eq:gan}) obtained on the last epoch. The hyperparameter $\lambda$ (right term in~\eqref{eq:gan}) was chosen from $\lambda \in \{0.1, 1.5, 3.5\}$.

\begin{table}[H]
    \centering
    \caption{Training parameters of the VAE models together with the values of the loss function \eqref{eq:vae} obtained at the last epoch.}
    \begin{tabular}{c|c|c|c|c}
         \textbf{index} & \textbf{latent size} $N_\alpha$ & $\beta$ & \textbf{KL loss} & \textbf{reconstruction loss}  \\
         \hline
         VAE1 & 2 & $\scnum{1.6e-02}$ & $1.5$ & $\scnum{2.1e-02}$ \\
         VAE2 & 2 & $\scnum{6.4e-03}$ & $2.5$ & $\scnum{1.1e-02}$ \\
         VAE3 & 2 & $\scnum{3.2e-03}$ & $3.4$ & $\scnum{6.7e-03}$ \\
         VAE4 & 3 & $\scnum{1.6e-02}$ & $1.5$ & $\scnum{2.1e-02}$ \\
         VAE5 & 3 & $\scnum{7.2e-03}$ & $2.4$ & $\scnum{1.1e-02}$ \\
         VAE6 & 3 & $\scnum{3.2e-03}$ & $3.5$ & $\scnum{5.5e-03}$ \\
         VAE7 & 6 & $\scnum{1.6e-02}$ & $1.5$ & $\scnum{2.1e-02}$ \\
         VAE8 & 6 & $\scnum{7.2e-03}$ & $2.4$ & $\scnum{1.1e-02}$ \\
         VAE9 & 6 & $\scnum{3.6e-03}$ & $3.3$ & $\scnum{6.0e-03}$ \\
    \end{tabular}
    \label{tabel:exp:vae}
\end{table}

\begin{table}[H]
    \centering
    \caption{Training parameters of the InfoGAN models together with values of the loss function \eqref{eq:gan} obtained at the last epoch. We report the generator loss (G loss), the information loss (I loss) and the total model loss (M loss).}
    \begin{tabular}{c|c|c|c|c|c}
         \textbf{Model} & \textbf{latent size} $N_\alpha$ & $\lambda$ & \textbf{G loss} & \textbf{I loss} & \textbf{M loss} \\
         \hline
         GAN1 & 2 & $0.1$ & $2.81$ & $0.10$ & $0.54$  \\
         GAN2 & 2 & $1.5$ & $2.28$ & $0.59$ & $0.78$ \\
         GAN3 & 2 & $3.5$ & $2.43$ & $1.07$ & $0.63$ \\
         GAN4 & 3 & $0.1$ & $2.52$ & $0.16$ & $0.61$ \\
         GAN5 & 3 & $1.5$ & $2.27$ & $1.45$ & $0.75$ \\
         GAN6 & 3 & $3.5$ & $2.23$ & $3.16$ & $0.68$ \\
         GAN7 & 6 & $0.1$ & $2.50$ & $0.44$ & $0.63$ \\
         GAN8 & 6 & $1.5$ & $2.23$ & $4.78$ & $0.73$ \\
         GAN9 & 6 & $3.5$ & $2.27$ & $10.32$ & $0.67$\\
    \end{tabular}
    \label{tabel:exp:gan}
\end{table}



\subsection{Evaluating the generative models}
\label{sec:exp:eval_gen_models}
We evaluated all the generative models using disentanglement, local linearity, precision and recall measures introduced in Section \ref{sec:eval_generative_model} as well as using the training parameters described in Tables~\ref{tabel:exp:vae} and~\ref{tabel:exp:gan}. We first studied the correlation of each individual evaluation measure and the performance of the policy training, and then the combined effect of all of the measures together. Our analysis empirically shows that any generative model having high recall improves the data-efficiency of the policy training task. Moreover, we observe that $\Dir$ is especially relevant in case of GANs, and precision in case of VAEs, while we do not find local linearity as essential for successful policy training. The details of our evaluation are presented and discussed in detail below.

%Our analysis empirically supports our hypothesis that a well disentangled, locally linear generative model that also possesses high precision and high recall improves the data-efficiency of the policy training task. Regardless of the type of the generative model, we identify recall as the most influential property followed by precision and disentangling recall $\Dir$. We observe that $\Dir$ is especially relevant in case of GANs, and precision in case of VAEs. The details of our evaluation are presented and discussed in detail below.



\textbf{EM policy training:}
\label{sec:exp:em_training}
For each generative model, introduced in Tables~\ref{tabel:exp:vae} and~\ref{tabel:exp:gan}, we trained one policy with three different random seeds. The obtained average training performances together with the standard deviations are shown in Figure~\ref{fig:exp:policy_training_performance}.  Using these results, we labeled each generative model with the
maximum reward achieved during EM policy training across all three random seeds. As it can be seen from Figure~\ref{fig:exp:policy_training_performance}, the best performance is achieved with VAE6 and VAE9 which have latent size $N_\alpha$ equal to 3 and 6, respectively, and low $\beta$ values.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{figures/policy_training_results.pdf}
\caption{A visualization of the performance of the policy training. We report the average reward together with the standard deviation ($y$-axis) obtained during EM policy training ($x$-axis) across three different random seeds. }
\label{fig:exp:policy_training_performance}
\end{figure}

We investigated the correlation between the characteristics of the generative models and the performance of the policy training in two different ways: (1) we calculated the Pearson's correlation between each \textit{individual} model characteristic and the corresponding model label introduced above, and (2) we studied the \textit{combined} effect that all of the properties have on the policy training using automatic relevance determination (ARD). We fit one ARD model for VAEs and GANs separately using the evaluation results discussed in the following and the training parameters from Tables \ref{tabel:exp:vae} and \ref{tabel:exp:gan} as inputs, and the policy performance as target values. Since ARD is sensitive to outliers, we additionally preprocessed the input values to the ARD using robust scaling with median and interquartile range. The results including Pearson's correlation coefficients (the higher, the better $\uparrow$) together with the corresponding p-values (the lower, the better $\downarrow$) as well as the ARD estimated precision of weights (the lower, the better $\downarrow$) are shown in Tables~\ref{tab:vae_pear_coef} and~\ref{tab:gan_pear_coef}. We first present the evaluation results and Pearson's correlations of each of the measures separately, and then discuss the differences with the ARD results.

% --- VAE Pearson's
\begin{table}[h]
    \centering
    \caption{Results for the correlation analysis of the VAE models to the policy performance. We report (1) Pearson correlation coefficient R (the higher, the better $\uparrow$) and (2) ARD estimated precision of the weights (the lower, the better $\downarrow$) between the evaluation metrics from Section \ref{sec:eval_generative_model} together with the training parameters from Table~\ref{tabel:exp:vae}, and the policy performance for VAE models visualised in Figure~\ref{fig:exp:policy_training_performance}.} 
    \vspace{0.2cm}
    \label{tab:vae_pear_coef}
    \begin{tabular}{r|c|c|c|c|c|c|c}
    & 
    \textbf{DiP} & \textbf{DiR} &
    \textbf{L3} & \textbf{Precision} & \textbf{Recall} & $\boldsymbol{N_\alpha}$ & $\boldsymbol{\beta}$
    \\
    \hline
    Pearson's R & 
    $0.600$ & 
    \cellcolor[gray]{0.94}{$0.668$} & 
    $-0.100$ & 
    \cellcolor[gray]{0.82}{$0.776$} &  \cellcolor[gray]{0.6}$0.969$ & $0.317$ & 
    \cellcolor[gray]{0.80}{$-0.791$} \\ 
        
    p-value & 
    $0.088$ &  \cellcolor[gray]{0.94}$0.049$ &  
    $0.797$ &  \cellcolor[gray]{0.82}$0.014$ &  \cellcolor[gray]{0.6}$0.000$ &  
    $0.406$ &  \cellcolor[gray]{0.8}$0.011$
    \\
    
    \hline
    ARD &  
    $\scnum{8.07e+04}$ &  $\scnum{1.81e+04}$ &  \cellcolor[gray]{0.8}$\scnum{1.09e+04}$ &  \cellcolor[gray]{0.7}$\scnum{4.45e+03}$ &  \cellcolor[gray]{0.60}$\scnum{1.93e+01}$ &  
    \cellcolor[gray]{0.9}$\scnum{1.70e+04}$ &  $\scnum{1.90e+04}$
    \end{tabular}
\end{table}

\begin{table}[h]
    \centering
    \caption{Results for the correlation analysis of the GAN models to the policy performance. We report (1) Pearson correlation coefficient R (the higher, the better $\uparrow$) and (2) ARD estimated precision of the weights (the lower, the better $\downarrow$) between the evaluation metrics from Section \ref{sec:eval_generative_model} together with the training parameters from Table~\ref{tabel:exp:gan}, and the policy performance for VAE models visualised in Figure~\ref{fig:exp:policy_training_performance}. } 
    \vspace{0.2cm}
    \label{tab:gan_pear_coef}
    \begin{tabular}{r|c|c|c|c|c|c|c}
    & 
    \textbf{DiP} & \textbf{DiR} & \textbf{L3} & \textbf{Precision} & \textbf{Recall} &  $\boldsymbol{N_\alpha}$ & $\boldsymbol{\lambda}$
    \\
    \hline
    Pearson's R & 
    $0.395$ &
    \cellcolor[gray]{0.82}$0.781$ &
    $-0.639$ &
    \cellcolor[gray]{0.80}$-0.801$ &  \cellcolor[gray]{0.65}$0.948$ &    \cellcolor[gray]{0.78}$0.823$ & 
    $0.368$  
    \\
    
    p-value & 
    $0.293$ &  \cellcolor[gray]{0.82}$0.013$ &  
    $0.064$ &  \cellcolor[gray]{0.80}$0.009$ &  \cellcolor[gray]{0.65}$0.000$ &  \cellcolor[gray]{0.78}$0.006$ &  
    $0.330$
    
    \\
    \hline
    ARD & \cellcolor[gray]{0.80}$\scnum{2.37e+02}$ &  \cellcolor[gray]{0.60}$\scnum{5.71e+01}$ &  $\scnum{3.20e+02}$ &  $\scnum{7.74e+02}$ &  \cellcolor[gray]{0.70}$\scnum{1.15e+02}$ &  
    \cellcolor[gray]{0.85}$\scnum{2.67e+02}$ &  $\scnum{5.50e+04}$ 
    \\
         
    \multicolumn{6}{c}{} \\
    &
    \textbf{G loss} & \textbf{I loss}&      \multicolumn{1}{c}{\textbf{M loss}}
    
    \\
    \cline{1-4}
    Pearson's R & 
    $-0.672$ & 
    $0.698$ & \multicolumn{1}{c}{$0.381$}
    
    \\
    p-value & 
    $0.048$ & 
    $0.036$ &  \multicolumn{1}{c}{$0.312$} 
    \\
    
    \cline{1-4}
    ARD & 
    $\scnum{4.66e+03}$ &  $\scnum{1.19e+05}$ &   \multicolumn{1}{c}{$\scnum{3.56e+02}$}
    \end{tabular}
\end{table}


% --- AGG figures are commented out
\begin{comment}
\begin{figure}[h]
\centering
\includegraphics[width=0.6\linewidth]{figures/AggIPR_nhood3_s5_n_samples15000.png}
\caption{Aggregated precision and recall scores.}\label{fig:ipr_agg}
\end{figure}
\end{comment}



\textbf{Disentanglement:}
We measured the disentangling precision and recall using $\MMD$ with kernel parameter $\gamma = 15$. For a given model $g$, we performed $D = 5$ interventions on every latent dimension $l \in \{1, \dots, N_\alpha\}$. 
We restricted the dimension of the end state space to $N_s = 3$ including only the position of the object and the angle of picking since these are the most relevant factors for performing the picking task.
The size of the sets $\boldsymbol{S}_g^{l-I_d}$ and $\boldsymbol{S}_r$ containing the end states was set to $n = 200$. For complete evaluation details we refer the reader to Appendix \ref{app:dis_score}. The obtained disentanglement scores are visualised in Figure \ref{fig:dis_all}. We observe that models with higher latent space dimension $N_\alpha$ (Figure \ref{fig:dis_all}, right) on average achieve higher disentangling recall $\Dir$. In Tables~\ref{tab:vae_pear_coef} and~\ref{tab:gan_pear_coef} we see that $\Dir$ is positively correlated to the performance of the policy, with a stronger correlation in case of GANs, while the positive correlation of $\Dip$ is not significant (p-value $> 0.05$). Therefore, when choosing  a generative model based only on disentanglement, it is beneficial that the interventions on the latent dimensions affect all three dimensions of the end state space. In other words, the latent action representations should capture all aspects of the robotic task, while it is less important to capture them precisely. 

% --- AGG figure is commented out
\begin{comment}
\begin{figure}[h]
\centering
\includegraphics[width=0.6\linewidth]{figures/MMDalpha15_AggDisentanglementScore_p0p001_paper.png}
\caption{Aggregated disentanglement scores.} \label{fig:dis_agg}
\end{figure}
\end{comment}

\begin{figure}[h]
\centering
\includegraphics[width=0.6\linewidth]{figures/MMDalpha15_disentanglementScore_p0p001_papernew.png}
\caption{Disentangling precision and recall scores for VAE models (top row) and GAN models (bottom row) with training parameters reported in Tables~\ref{tabel:exp:vae} and \ref{tabel:exp:gan}, respectively.} \label{fig:dis_all}
\end{figure}
 
\textbf{Local linearity:}
Given a generative model $g$, we randomly sampled $50$ latent actions from the prior $p(\alpha)$. For each such latent action $\alpha$, we set $\varepsilon = 0.2$ and sampled $500$ points from its $\varepsilon$-neighbourhood $N_\varepsilon(\alpha)$. We then fit an affine transformation $f_\alpha$ defined in~\eqref{eq:aff_trans} on $350$ randomly selected neighbourhood points and calculated L3 as the test MSE on the remaining $150$ points. We report the average test MSE obtained across all $50$ points in Table~\ref{tabel:exp:loclin}. We observe that all VAEs except for VAE3 achieve a lower test MSE than GAN models. By comparing Figure~\ref{fig:exp:policy_training_performance} and Table~\ref{tabel:exp:loclin} it appears that local linearity is not related to the performance of the policy training which is on par with the results obtained in 
Tables~\ref{tab:vae_pear_coef} and~\ref{tab:gan_pear_coef} where we see that the correlation is not significant neither for VAEs nor for GANs. Despite being insignificant, the correlation is negative for all the models which coincides with our hypothesis that a more locally linear model (i.e., a model with a lower MSE) performs better in the policy training.
 
%\begin{figure}[h]
%\centering
%\includegraphics[width=0.6\linewidth]{figures/test_MSE_vae_0_2_npoints50times500_new.png}
%\caption{Local linearity test MSE.} \label{tabel:exp:loclin}
%\end{figure}

\begin{table}[H]
    \centering
    \caption{The Latent Local Linearity (L3) results measured as the mean squared error (MSE) of the affine transformations defined in~\eqref{eq:aff_trans} in the neighbourhoods of 50 latent action representations for all VAE and GAN models.}
    \vspace{0.2cm}
    \begin{tabular}{c c c c c c c c c c}
         \textbf{Model} & VAE1 & VAE2 & VAE3 & VAE4 & VAE5 & VAE6 & VAE7 & VAE8 & VAE9  \\
         \hline
         \textbf{MSE} & 1.6& 3.2& 14.3& 1.5& 1.6& 2.0& 1.2& 1.2& 1.3\\
         & &  &  &  &  &  &  &  & \\
         \textbf{Model}&GAN1 & GAN2 & GAN3 &GAN4 & GAN5 & GAN6 &GAN7 & GAN8 & GAN9\\
         \hline
         \textbf{MSE} &73.1&27.8&41.1&16.7&36.6&43.0&14.2&24.7&5.2 \\
    \end{tabular}
    \label{tabel:exp:loclin}
\end{table}


\textbf{Precision and recall:}
For each generative model $g$, we randomly sampled $15000$ samples from the latent prior distribution $p(\alpha)$. The corresponding set of the generated trajectories $\boldsymbol{T_g}$ was compared to a set $\boldsymbol{T_r}$ of $15000$ randomly chosen training trajectories  which were sampled only once and fixed for all the models. The neighbourhood size $k$ was set to $3$ as suggested in \cite{kynkaanniemi2019improved}. The resulting precision and recall scores are shown in Figure \ref{fig:ipr_all}. Firstly, we observe that all the models have relatively high precision except for GAN8-9 which are shown in the bottom right part of Figure~\ref{fig:ipr_all}. Secondly, on average GANs have worse recall than VAEs, which is a consequence of the training procedure (see Appendix \ref{app:gen_models}) and can possibly be improved with a more thorough fine tuning of the models. This is consistent with the results reported in Table~\ref{tab:gan_pear_coef} where precision is negatively correlated to the policy performance in case of GANs but positively in case of VAEs. For both VAE and GAN models, we observe that recall is highly correlated with the performance of the policy training.

%we obtained a negative correlation of precision measure in case of GANs, while the correlation is positive for the VAEs. 
 
\begin{figure}[h]
\centering
\includegraphics[width=0.6\linewidth]{figures/IPR_nhood3_s5_n_samples15000_new.png} %\label{fig:ipr_all}
\caption{Precision and recall scores for VAE (top row) and GAN models (bottom row).}\label{fig:ipr_all}
\end{figure}
 

\textbf{Training parameters:} In Tables~\ref{tab:vae_pear_coef} and~\ref{tab:gan_pear_coef} we additionally calculated the Pearson's correlation between the training parameters, shown in Tables~\ref{tabel:exp:vae} and~\ref{tabel:exp:gan}, and the policy performance shown in Figure~\ref{fig:exp:policy_training_performance}. For VAEs, we used only the $\beta$ coefficient as it is clearly correlated with the KL divergence and the reconstruction loss (see Table~\ref{tabel:exp:vae}). Interestingly, we observe negative correlation between $\beta$ and policy training performance which indicates that  disentangled representations are less beneficial as these are obtained with a higher $\beta$ value. This observation is also supported by a low Pearson's coefficient obtained for $\Dir$ and insignificant correlation of $\Dip$ (see Table~\ref{tab:vae_pear_coef}). In fact, increasing $\beta$ positively affects the disentanglement as shown in~\cite{higgins2017beta} on image data, but negatively the precision, because data is in this case reconstructed from a wider approximate posterior distribution $q_\varphi$. Since precision is more important for an efficient policy performance than disentanglement in case of VAEs, the correlation of $\beta$ is negative.
Next, a positive correlation of the latent dimension $N_\alpha$ is observed for both VAE and GAN models but for VAEs it is insignificant. Finally, the correlation coefficients for GAN losses imply that the lower the generator loss (G loss) and the higher the information loss (I loss), the better the policy performance. This result is meaningful as higher I loss, obtained with a higher $\lambda$, encourages more disentangled representations, which we also see with a high $\Dir$ correlation coefficient. 

%So far, we have discussed the relation of each individual characteristic of generative models with the performance of the policy. Next, we investigated the combined effect that all of the properties have on the policy training using automatic relevance determination (ARD) framework.

\textbf{Correlation between evaluation metrics and EM policy training:} Possibly due to the sensitivity of the ARD framework to outliers, the obtained ARD results shown in Tables~\ref{tab:vae_pear_coef} and \ref{tab:gan_pear_coef} differ slightly from the Pearson's R correlation coefficients. In case of VAEs, local linearity seems to be more important due to the large outlying value for the VAE3 model (Table~\ref{tabel:exp:loclin}). Similarly, $\Dip$ appears to be influential in case of GANs due to the large range of values (Figure
~\ref{fig:dis_all} left). For both model types, ARD analysis shows $N_\alpha$ to be important which can also be a consequence of the chosen values $N_\alpha \in \{2, 3, 6\}$. However, ARD scores precision and recall as influential in case of VAEs, as well as $\Dir$ and recall in case of GANs, both of which matches the Pearson's correlation results.
 
%We first fit one ARD model for VAEs and GANs separately. We used the results presented above as well as the training parameters from Tables~\ref{tabel:exp:vae} and~\ref{tabel:exp:gan} as inputs, and the policy performance as target values. Since ARD is sensitive to outliers, we preprocessed the input values using robust scaling with median and interquartile range. The resulting estimated precision of the weights (the lower, the better $\downarrow$)  corresponding to the properties of the generative models are reported in Tables \ref{tab:vae_ard_coef} and~\ref{tab:gan_ard_coef}. 
%For VAEs (Table~\ref{tab:vae_ard_coef}), we see that the most influential properties for predicting the performance of the policy are recall and precision, while local linearity, $N_\alpha$, $\Dir$, $\beta$ and $\Dip$ are of secondary importance (listed in the order of importance). The observed ARD results coincide well with the individual correlations shown in Table~\ref{tab:vae_pear_coef}, with minor deviations that occur due to the ARD model seeking for features with strongest predictive power. For instance, we observed significant correlation for both $\Dir$ and $\beta$ (Table~\ref{tab:vae_pear_coef}) but they appear to be less important in the ARD model.
\begin{comment}
\begin{table}[h]
    \centering
    \caption{ARD estimated precision (the lower, the better $\downarrow$) of the weights   corresponding to the evaluation metrics from Section \ref{sec:eval_generative_model} and training parameters for VAE models.}
    \vspace{0.2cm}
    \label{tab:vae_ard_coef}
    \begin{tabular}{c|c|c|c|c|c|c}
          \textbf{DiP} & \textbf{DiR} & \textbf{L3} &\textbf{Precision} & \textbf{Recall} 
          & $\boldsymbol{N_\alpha}$
          & $\boldsymbol{\beta}$
          \\
         \hline
         %mean, sta & $\scnum{4.61e+02}$ &  $\scnum{9.21e+04}$ &  $\scnum{4.05e+02}$ &  $\scnum{4.86e+03}$ &  $\scnum{1.83e+02}$ &  $\scnum{3.90e+05}$ &  $\scnum{1.14e+04}$ %$\scnum{5.24e+01}$ &  $\scnum{1.36e+04}$ &  $\scnum{4.45e+01}$ &  $\scnum{6.99e+02}$ &  $\scnum{2.10e+01}$ &  $\scnum{6.70e+04}$ &  $\scnum{2.83e+04}$ \\mean, robust &  $\scnum{4.38e+04}$ &  $\scnum{1.20e+04}$ &  $\scnum{1.27e+04}$ &  $\scnum{2.57e+02}$ &  $\scnum{2.51e+01}$ &  $\scnum{1.23e+05}$ &  $\scnum{1.39e+04}$ \\max, standard & $\scnum{2.99e+02}$ &  $\scnum{1.96e+04}$ &  $\scnum{3.18e+02}$ &  $\scnum{4.18e+04}$ &  $\scnum{1.04e+02}$ &  $\scnum{2.43e+04}$ &  $\scnum{1.63e+04}$ \\
         $\scnum{8.07e+04}$ &  $\scnum{1.81e+04}$ &  \cellcolor[gray]{0.85}$\scnum{1.09e+04}$ &  \cellcolor[gray]{0.75}$\scnum{4.45e+03}$ &  \cellcolor[gray]{0.65}$\scnum{1.93e+01}$ &  
         $\scnum{1.70e+04}$ &  $\scnum{1.90e+04}$ %$\scnum{3.32e+01}$ &  $\scnum{3.82e+04}$ &  $\scnum{3.53e+01}$ &  $\scnum{1.22e+04}$ &  $\scnum{1.16e+01}$ &  $\scnum{1.03e+04}$ &  $\scnum{1.40e+04}$
    \end{tabular}
\end{table} 

For GANs (Table~\ref{tab:gan_ard_coef}), we observe that several more properties are important for forecasting the performance of the policy than in case of VAEs, namely $\Dir$, recall, $\Dip$, $N_\alpha$, local linearity, the total model loss (M loss) and lastly local linearity (listed in the order of importance). Similarly as for VAEs, we see that the ARD results are well aligned with the individual correlations shown in Table~\ref{tab:gan_pear_coef}, however, we observe slightly larger deviations than with VAEs. For example, while we did not observe a significant correlation of $\Dip$, local linearity and model loss to the policy performance, these properties gain importance in the ARD model. On contrary, the observed significant correlation of the generator loss (G loss) as well as the information loss (I loss) appear to be too weak for the ARD model.

\begin{table}[h]
    \centering
    \caption{ARD estimated precision (the lower, the better $\downarrow$) of the weights   corresponding to the evaluation metrics from Section \ref{sec:eval_generative_model} and training parameters for GAN models.}
    \vspace{0.2cm}
    \label{tab:gan_ard_coef}
    \begin{tabular}{c|c|c|c|c|c|c}
          \textbf{DiP} & \textbf{DiR} &
          \textbf{L3}
          & \textbf{Precision} & \textbf{Recall} &  $\boldsymbol{N_\alpha}$
          & $\boldsymbol{\lambda}$
          \\
         \hline
         \cellcolor[gray]{0.85}$\scnum{2.37e+02}$ &  \cellcolor[gray]{0.65}$\scnum{5.71e+01}$ &  
         $\scnum{3.20e+02}$ &  $\scnum{7.74e+02}$ &  \cellcolor[gray]{0.75}$\scnum{1.15e+02}$ &  
         $\scnum{2.67e+02}$ &  $\scnum{5.50e+04}$ 
         \\
         \multicolumn{7}{c}{} \\
         \textbf{G loss} & \textbf{I loss}&      \multicolumn{1}{c}{\textbf{M loss} }\\\cline{1-3}$\scnum{4.66e+03}$ &  $\scnum{1.19e+05}$ &   \multicolumn{1}{c}{$\scnum{3.56e+02}$}
    \end{tabular}
\end{table}
\end{comment}

Lastly, we wished to compare all the generative models only based on the properties that can be evaluated for both model types. Therefore, we fit three ARD models, one for VAEs, one for GANs and one for all the models combined using only $\Dip$, $\Dir$, local linearity, precision and recall. The obtained estimated precision of the weights are reported in Table~\ref{tab:ard_coef}. While we observe minor differences between the two model types, we see that the most important property of a generative model combined with EM policy training is recall which is consistent with the results obtained in Tables
~\ref{tab:vae_pear_coef} and \ref{tab:gan_pear_coef}. Similarly as before, disentangling precision $\Dip$ gains importance due to the large range of values (Figure~\ref{fig:dis_all}). Therefore, for successful policy training in case of the picking task, it is crucial that the generative model is able to reproduce samples from the training dataset even if the generated samples are less precise. Based on the observations from Tables
~\ref{tab:vae_pear_coef} and \ref{tab:gan_pear_coef} we conclude that GAN models additionally benefit from a higher disentangling recall $\Dir$, while VAEs benefit from a higher precision. Finally, we note that disentangling precision as well as local linearity can become more important when performing tasks represented by more complex data where structured latent representations would be beneficial.

%, followed by precision and disentangling precision $\Dip$, while disentangling recall $\Dir$ and local linearity are less important. Therefore, for a successful policy training in case of the picking task, it is crucial that the generative model is able to reproduce samples from the training dataset even if the generated samples are less precise. Due to the large range of values for $\Dip$ (see Figure~\ref{fig:dis_all}), we observe $\Dip$ gained more importance than $\Dir$ in the ARD model. Since this is an artifact of the ARD framework, we conclude based on our earlier observations that the latent representations should be well disentangled where higher disentangling recall $\Dir$ is more beneficial for a successful policy training than higher disentangling precision $\Dip$. We observe that local linearity in general has a low effect on the policy performance although this can vary with the choice of the generative model. Finally, we note that disentanglement and local linearity can be essential when performing tasks represented by more complex data such that structured latent representations would be beneficial.

\begin{table}[h]
    \centering
    \caption{ARD estimated precision of the weights (the lower, the better $\downarrow$) corresponding to the evaluation metrics from Section \ref{sec:eval_generative_model} for all the VAE and GAN models.}     
    \vspace{0.2cm}
    \label{tab:ard_coef}
    \begin{tabular}{r|c|c|c|c|c}
        \textbf{models} 
          & \textbf{DiP} & \textbf{DiR}
          & \textbf{L3}  
          & \textbf{Precision} & \textbf{Recall}   \\
         \hline
          VAEs & \cellcolor[gray]{0.75}$\scnum{2.78e+02}$ &  
          $\scnum{1.83e+04}$ 
          &  
          \cellcolor[gray]{0.85}$\scnum{9.42e+03}$ &  
          $\scnum{2.24e+04}$ 
          &  
          \cellcolor[gray]{0.65}$\scnum{3.56e+01}$
         \\
         \hline
         GANs & \cellcolor[gray]{0.75}$\scnum{8.17e+02}$ &  
         \cellcolor[gray]{0.85}$\scnum{1.09e+04}$ &  
         $\scnum{1.25e+04}$ &  $\scnum{3.97e+04}$ &  
         \cellcolor[gray]{0.65}$\scnum{2.66e+01}$ \\
         \hline
         
         ALL & \cellcolor[gray]{0.75}$\scnum{3.62e+03}$ &  
         $\scnum{1.60e+04}$ & $\scnum{1.51e+04}$ 
         &  
         \cellcolor[gray]{0.85}$\scnum{6.27e+03}$ & 
         \cellcolor[gray]{0.65}$\scnum{3.45e+01}$
          \\
          
         
    \end{tabular}
\end{table}


% ------ 
% Removed experiments for several variatonal policies cause they are not strong enough
\begin{comment}
\textbf{EM policy training with multiple variational policies:}
Figure~\ref{fig:exp:multi_agent} demonstrates the performance of the EM policy training algorithm for different numbers of variational policies in the E-step.
We see that using more than one variational policy in the E-step improves the performance in the beginning of the training since the RL agent learns faster with more than 4 variational policies for the first 100 iterations. 
However, the best performance is still achieved by the EM policy training with one variational policy. 
This observation requires more investigations which is a part of our future work. 

\begin{figure}[h]
\centering
\includegraphics[width=0.5\linewidth]{figures/multi_agent_res.pdf}
\caption{The performance of the EM policy training for 1, 2, 4, and 8 variational policies. The results are obtained using VAE9 whose parameters are described in Table~\ref{tabel:exp:vae}.}
\label{fig:exp:multi_agent}
\end{figure}
\end{comment}


%\subsection{End-to-end policy training on the real robot hardware}
%\label{sec:exp:end-to-end}




==> original/inputs/generative_model_training.tex <==
\section{Generative Model Training}
\label{sec:generative_model_training}
So far we discussed how to train an action-selection policy based on the EM algorithm to regulate the action latent variable which is the input to a generative model. % to generate proper action sequences in different contexts, i.e., different states of the system. 
In this section, we review two prominent approaches to train a generative model, Variational Autoencoder (VAE) and Generative Adversarial Network (GAN), which we use to generate sequences of actions required to solve the sequential decision-making problem. 
%We then discuss which properties of generative models are necessary to ensure an efficient policy training and 
We then introduce a set of measures used to predict which properties of a generative model will influence the performance of the policy training. 

\subsection{Training generative models}
We aim to model the distribution $p(\tau)$ of the motor actions  that are suitable to complete a given task. To this end, we introduce a low-dimensional random variable $\alpha$ with a probability density function $p(\alpha)$ representing the latent actions which are mapped into unique trajectories $\tau$ by a generative model $g$. The model $g$ is trained to maximize the likelihood $\mathbb{E}_{\tau \sim \mathcal{D}, \alpha' \sim p(\alpha)}[p_\vartheta(\tau|\alpha')]$ of the training trajectories $\tau \in \mathcal{D}$ under the entire latent variable space.
%In fact, the generative model is the deterministic version of $p(\tau|\alpha)$, i.e., $\tau \leftarrow g(\alpha)$ by using the mean of the distribution.

\subsubsection{Variational autoencoders}
A VAE \cite{kingma2014auto, rezende2014stochasticvae2} consists of encoder and decoder neural networks representing the parameters of the approximate posterior distribution $q_\varphi(\alpha | \tau)$ and the likelihood function $p_\vartheta(\tau|\alpha)$, respectively. The encoder and decoder neural networks, parametrized by $\varphi$ and $\vartheta$, respectively, are jointly trained to optimize the variational lower bound
\begin{equation}
     \max_{\varphi, \vartheta} \mathbb{E}_{\alpha' \sim q_\varphi(\alpha|\tau)}[\log p_\vartheta(\tau|\alpha')] - \beta D_{KL}(q_\varphi (\alpha | \tau) || p(\alpha)),
\label{eq:vae}
\end{equation}
where the prior $p(\alpha)$ is the standard normal distribution and the parameter $\beta$ \cite{higgins2017beta} a variable controlling the trade-off between the reconstruction fidelity and the structure of the latent space regulated by the KL divergence. A $\beta > 1$ encourages the model to learn more disentangled latent representations \cite{higgins2017beta}.

\subsubsection{Generative adversarial networks}
A GAN model \cite{goodfellow2014generative} consists of a generator and discriminator neural networks that are trained by playing a min-max game. The generative model $g_\vartheta$, parametrized by $\vartheta$, transforms a latent sample $\alpha'$ sampled from the prior noise distribution $p(\alpha)$ into a trajectory $\tau = g_\vartheta(\alpha')$. The model needs to produce realistic samples resembling those obtained from the training data distribution $p(\tau)$. It is trained by playing an adversarial game against the discriminator network $D_\varphi$, parametrized by $\varphi$, which needs to distinguish a generated sample from a real one. The competition between the two networks is expressed as the following min-max objective
\begin{align}
    \min_\vartheta \max_\varphi \mathbb{E}_{\tau' \sim p(\tau)} [\log D_\varphi(\tau')] + \mathbb{E}_{\alpha' \sim p(\alpha)} [\log(1 - D_\varphi(g_\vartheta(\alpha'))]. \label{eq:gan_original}
\end{align}
However, the original GAN formulation~\eqref{eq:gan_original} does not impose any restrictions on the latent variable $\alpha$ and therefore the generator $g_\vartheta$ can use $\alpha$ in an arbitrary way. To learn disentangled latent representations %Since our hypothesis is that better disentangled latent representations lead to more efficient RL policy training, 
we instead use InfoGAN \cite{chen2016infogan} which is a version of GAN with an information-theoretic regularization added to the original objective. The regularization is based on the idea to maximise the mutual information $I(\alpha', g_\vartheta(\alpha'))$ between the latent code $\alpha'$ and the corresponding generated sample $g_\vartheta(\alpha')$. %which encourages the latent representation to be disentangled. 
An InfoGAN model is trained using the following information minmax objective \cite{chen2016infogan}
%The authors in \cite{chen2016infogan} derive the following lower bound for the information objective
\begin{equation}
    \min_{\vartheta, \psi} \max_\varphi \mathbb{E}_{\tau' \sim p(\tau)} [\log D_\varphi(\tau')] + \mathbb{E}_{\alpha' \sim  p(\alpha)} [\log(1 - D_\varphi(g_\vartheta(\alpha'))] - \lambda \mathbb{E}_{\alpha' \sim p(\alpha), \tau' \sim g_\vartheta(\alpha')}[\log Q_\psi(\alpha' | \tau')],
\label{eq:gan}
\end{equation}
where $Q_\psi(\alpha | \tau')$ is an approximation of the true unknown posterior distribution $p(\alpha | \tau')$ and $\lambda$ a hyperparameter. In practice, $Q_\psi$ is a neural network that models the parameters of a Gaussian distribution and shares all the convolutional layers with the discriminator network $D_\varphi$ except for the last few output layers.


%\subsubsection{Collecting motion trajectory data}
%In general, it is not challenging to find a set of motion trajectories that are suitable to complete a given task. 
%The trajectories do not need to consider a goal state to reach nor to take the dynamics of the task into account. The only assumption is that there exists an arbitrary goal state which is reachable given the robot motion trajectory.
%The training trajectories $\mathcal{D_\tau}$ for each task can be collected using human kinestatic demonstrations,
%general path planning frameworks, e.g., rapidly-exploring random tree RRT* \cite{karaman2010incremental}, 
%physics-based rules, e.g., \cite{zeng2019tossingbot}, blind controllers without a target state, e.g., \cite{ghadirzadeh2017deep,finn2016deep}, or in simulation. 

%The benefit of representing the motion trajectories using the generative model compared to path planning methods or hand-engineered controllers is that it gives more freedom to formulate the solution as a data-driven approach. The neural network architecture of the generative model enables end-to-end training with the possibility of incrementally improving the performance as more data is collected. 
%Using the neural network generative models facilitates policy search even for kinodynamic tasks, e.g., throwing objects \cite{ghadirzadeh2017deep}, or hitting objects to slide as shown in our experiments. 


\subsection{Evaluation of the generative models}
\label{sec:eval_generative_model}
We review the characteristics of generative models that can potentially improve the policy training by measuring precision and recall, disentanglement and local linearity. Our goal is to be able to judge the quality of the policy training by evaluating the generative models prior to the RL training. We relate the measures to the performance of the policy training in Section~\ref{sec:exp:generative_model}. 


\begin{comment}
The authors in \cite{sajjadi2018assessing} define a learned distribution $Q$ to have precision $\alpha$ at recall $\beta$ with respect to the reference distribution $P$ if there exist distributions $\mu, \nu_P$ and $\nu_Q$ such that $P$ and $Q$ can be decomposed as follows:
\begin{align}
    P = \beta \mu + (1 - \beta) \nu_P \quad \text{and} \quad Q = \alpha \mu + (1 - \alpha) \nu_Q. \label{def:prd_1}
\end{align}
The distribution $\mu$ models the part common to both the reference distribution $P$ as well as the learned distribution $Q$. The distribution $\nu_P$ represents the part of $P$ that $Q$ does not cover, and $\nu_Q$ represent the part of $Q$ that is irrelevant for $P$, in the sense that its support does not intersect the support of the reference distribution. The precision-recall curve can then be obtained by visualising the set $\PRD(P, Q) = \{(\alpha, \beta): \alpha, \beta \text{ satisfying Eq. \eqref{def:prd_1}}\}$. However, this definition is difficult to work with in practice as it requires an estimation of distributions $\mu, \nu_P, \nu_Q$ for every possible pair $(\alpha, \beta)$. Therefore, the authors provide an approximation that is based only on evaluation of $P$ and $Q$ on finite number of samples:
\begin{align*}
    \alpha(\lambda) = \sum_{\omega \in \Omega} \min(\lambda P(\omega), Q(\omega)) \quad \text{and} \quad \beta(\lambda) = \sum_{\omega \in \Omega} \min \left( P(\omega), \frac{Q(\omega)}{\lambda} \right) 
\end{align*}
where $\lambda > 0$ and $\Omega$ is the state space where $P$ and $Q$ are defined. Intuitively, the function $\alpha(\lambda)$ will be non-negative only on samples $\omega \in \Omega$ where $Q$ is non-negative. On such samples, it then measures how much we need to change the reference distribution $P$ in order to be close to $Q$. This is exactly the precision of $Q$: it will be low if $Q$ deviates from $P$ on the support of $Q$. On the other hand, the function $\beta(\lambda)$ will be non-negative only on samples $\omega \in \Omega$ where $P$ is non-negative. By measuring the difference between $P$ and $Q$ on such samples, we obtain an approximation of the recall: it will be low if $Q$ is zero on the support of $P$. The final approximation of the $\PRD$ set can then be computed by evaluating the functions $\alpha$ and $\beta$ on an equiangular grid of values $\lambda$:
\begin{align*}
    \widehat{\PRD}(Q, P) = \left\{ (\alpha(\lambda), \beta(\lambda)): \lambda \in \left\{\tan\left(\frac{i \pi}{2(m+1)}\right)\right\}_{i=1}^m \right\}.
\end{align*}
In our experiments, we use the original implementation of this algorithm provided by the authors of \cite{sajjadi2018assessing}.
\end{comment}


\subsubsection{Disentangling precision and recall}
In this section, we define our measure, called \textit{disentangling precision and recall,} for evaluating the disentanglement of latent action representations. 
%Disentangled representations obtained through unsupervised representation learning 
%have shown to improve the learning efficiency of a large variety of downstream machine learning tasks \cite{bengio2013representation, chen2016infogan, higgins2017beta}. 
%We define representation of the motor data obtained from the latent space of a generative model as disentangled if every end state of the system is controllable by one latent dimension. 
A disentangled representation of the motor data obtained from the latent space of a generative model can be defined as the one in which every end state of the system is controllable by one latent dimension determined by the vector basis of the latent space. 
For example, consider the picking task where the goal is to pick an object on a table top (Section~\ref{sec:exp:setup}). We say that a latent representation given by a generative model is well-disentangled if there exists a basis of the latent space with respect to which each dimension controls one axis of the position of the end-effector.
%A well-disentangled representation given by a generative model forces each axis of the position of the end-effector to be controlled by one dimension of the latent variable. 
Our hypothesis is that the more disentangled the representation is, the more efficient is the policy training. 
While disentangled representations have been successfully applied to a variety of downstream machine learning tasks \cite{disentanglement_video, creager2019flexibly, lee2018diverse}, their usefulness has been questioned by \cite{challenging_common} and \cite{van2019disentangled} who have observed disagreements among the existing disentanglement metrics. 
We experimentally evaluate the effect of disentangled representations on the performance of the policy training in Section~\ref{sec:exp:eval_gen_models}.

%The existing metrics for measuring disentanglement \cite{higgins2017beta, kim2018disentangling, eastwood2018framework, chen2018isolating} rely on the prior knowledge of the ground truth factors of variation given in the dataset as they are based on measuring how changes in the generative factors of the dataset affect the latent representations. 
%Such requirement is not likely to be fulfilled by real world datasets which is the case in the motor data as well. 
%Moreover, these frameworks are typically developed on image data where it is possible to validate the metrics by either a visual inspection of the generated samples or, in the case when labeled data is available, by relying on an external classifier. Such approaches are not feasible in the case of the motor data as it is difficult to define what are ground truth factors of variation, to provide labels, or to visualise it. However, in this case we do have access to the end state of the system that corresponds to a given latent representation. We can therefore evaluate the disentanglement in an unsupervised manner without the above requirements by measuring how changes in the latent space affect the obtained end states. 

%The idea of our disentanglement measure is based on quantifying the difference between the distribution of the end states obtained from a trained generative model and the distribution of the end states of the ground truth motor data. 

Our disentanglement measure is based on statistical testing performed on the end state space of the system.
%Let $\boldsymbol{S}_r$ and $\boldsymbol{S}_g$ be the sets of end states obtained by executing the training motor trajectories and the trajectories generated by the generative model $g$, respectively. 
Let $\boldsymbol{S}_r$ be the set of end states obtained by executing the training motor trajectories on a robotic platform. If representations given by $g$ are well disentangled, then setting one latent dimension to a fixed value should result in limited variation in the corresponding generated end states $\boldsymbol{S}_g$. For example, if the $1$st latent dimension controls the $x$-axis position of the end-effector in the picking task then setting it to a fixed value should limit the set of possible $x$ positions. %To determine if there exist such correlations between the latent dimensions and the components of the end states, we %compare the sets $\boldsymbol{s}_r$ and $\boldsymbol{s}_g$
%the end states obtained by a generative model with the ground truth end states 
In other words, we wish to quantify how dissimilar the set of end states $\boldsymbol{S}_g$, obtained by holding one latent dimension constant, is from the set $\boldsymbol{S}_r$. To compute such dissimilarity we use maximum mean discrepancy (MMD) \cite{JMLR:v13:gretton12a} which is a statistical test for determining if two sets of samples were produced by the same distribution. Using kernels, MMD maps both sets into a feature space called reproducing kernel Hilbert space, and computes the distance between mean values of the samples in each group. In our implementations, we compute the unbiased estimator of the squared MMD (Lemma 6 in \cite{JMLR:v13:gretton12a}) given by 
\begin{align*}
    \text{MMD}^2(\boldsymbol{S}_r, \boldsymbol{S}_g) = \frac{1}{m (m -1)} \sum_{i \neq j}^m k(s_r^i, s_r^j) + \frac{1}{n (n -1)} \sum_{i \neq j}^n k(s_g^i, s_g^j) - \frac{2}{mn} \sum_{i = 1}^m \sum_{j = 1}^n k(s_r^i, s_g^j),
\end{align*}
where, $\boldsymbol{S}_r = \{s_r^1, \dots, s_r^m\}$, $\boldsymbol{S}_g = \{s_g^1, \dots, s_g^n\}$ are the two sets of samples and $k(x, y) = \exp(- \gamma ||x - y||^2)$ is the exponential kernel with hyperparameter $\gamma$ determining the smoothness. Due to the nature of the exponential kernel, the higher the MMD score, the lower the similarity between the two sets.
 
Our measure can be described in three phases. We provide an intuitive summary of each phase but refer the reader to Appendix \ref{app:dis_score} for a rigorous description of the algorithm. In phase $1$ (Figure \ref{fig:disentanglement_graphics} left) we generate the two sets of end states on which we run the statistical tests. For a fixed latent dimension $l \in \{1, \dots, N_\alpha\}$ we perform a series of $D \in \mathbb{N}$ \textit{latent interventions} where we set the $l$th component of a latent code $\alpha_l$ to a fixed value $I_d$, $\alpha_l = I_d$ for $d = 1, \dots, D$. Each intervention $\alpha_l = I_d$ is performed on a set of $n$ samples sampled from the prior distribution $p(\alpha)$. We denote by $\boldsymbol{S}_g^{l-I_d}$ the set of $n$ end states obtained by executing the trajectories generated from the latent samples on which we performed the intervention $\alpha_l = I_d$. For example, $D = 5$ latent interventions on the $1$-st latent dimension yield the sets $\boldsymbol{S}_g^{1-I_1}, \dots, \boldsymbol{S}_g^{1-I_5}$. Moreover, we denote by $\boldsymbol{S}_r$ the set of $n$ randomly subsampled end states that correspond to the training motor data.  

\begin{figure}[h]
\centering
\includegraphics[width=0.99\linewidth]{figures/disentanglement_graphics.png}
\caption{Visualisation of phase 1 and 2 of our disentangling precision and recall metric $\Dis$. }\label{fig:disentanglement_graphics}
\end{figure}

In phase $2$ (Figure \ref{fig:disentanglement_graphics} right), we perform the $\MMD$ tests on each pair of sets $\boldsymbol{S}_g^{l-I_d}$ and $\boldsymbol{S}_r$ obtained in phase $1$. In particular, we wish to determine if an intervention on a given dimension $l$ induced a change in any of the components $j = 1, \dots, N_s$ of the end state space. If such a change exists, we consider the latent dimension $l$ to be well disentangled. Moreover, if we can find a set of latent dimensions that induce changes on different components of the end states, we consider the generative model $g$ to be well disentangled. Therefore, for a fixed latent dimension $l$ and a fixed intervention $\alpha_l = I_d$, the objective is to find the component $j$ of the end state space for which $\boldsymbol{S}_g^{l-I_d}$ and $\boldsymbol{S}_r$ are most dissimilar. This translates to finding the component $j$
yielding the largest 
value $\MMD(\proj_j \boldsymbol{S}_g^{l-I_d}, \proj_j \boldsymbol{S}_r)$  where $\proj_j \boldsymbol{S} = \{ \proj_j s \,|\,s \in \boldsymbol{S} \}$ denotes the set of the $j$th components of the states from the set $\boldsymbol{S}$. Note that if the dimension $l$ is entangled such component $j$ does not exists (see Appendix \ref{app:dis_score} for details). 

In phase $3$ we aggregate the values of the performed $\MMD$ tests and define the final disentanglement score for the generative model $g$. In phase $2$ we linked each latent dimension $l$ with zero or one end state component $j$, and computed the corresponding value of the $\MMD$ test. Here, we first select $\min(N_s, N_\alpha)$ such pairs of latent space and end state space dimensions that yield the largest $\MMD$ values. In other words, we select the latent dimensions for which the latent interventions resulted in the largest changes in the end state space. We define $\Dip(g)$ as the sum of the selected $\MMD$ values, and $\Dir(g)$ as the number of unique end state space components present in the selected pairs, normalised by the total number of components $N_s$. Finally, we define the \textit{Disentangling Precision and Recall} $\Dis$ as a pair $$\Dis(g) = (\Dip(g), \Dir(g)).$$
Intuitively, $\Dip(g)$ quantifies the sum effect of the latent interventions with the most impact on the end states, and can therefore be thought of as \textit{disentangling precision}. A high $\Dip$ value indicates that the intervened latent samples resulted in end states with significantly limited variation, which in turn means that the latent disentanglement has a high precision. On the other hand, $\Dir(g)$ measures how many different aspects of the end states are captured in the latent space, and can be thus thought of as \textit{disentangling recall}. A high $\Dir$ value indicates that more end state components are captured in the latent space, such that the latent disentanglement has a high recall. The defined score is a novel fully unsupervised approximate measure of disentanglement for generative models combined with the RL policy training. Its absolute values can however vary depending on the kernel parameter $\gamma$ determining its smoothness. Moreover, this measure is not to be confused with the precision and recall from Section \ref{sec:prec_and_recall} where the aim is to evaluate the quality of the generated samples as opposed to the quality of the latent representations.


\subsubsection{Latent Local linearity}
The linearity of system dynamics plays a vital role in control theory but has not been studied in the context of generative model training. 
The system dynamics govern the evolution of the states as the result of applying a sequence of motor actions to the robot. Our hypothesis is that a generative model integrated with the environment performs better in the policy training if it satisfies the local linearity property defined below.

Let the mapping $\text{Exe}: \mathbb{R}^{T \times M} \rightarrow \mathbb{R}^{N_s}$ correspond to the execution of motion actions on a robot and let $s = \text{Exe}(\tau) \in \mathbb{R}^{N_s}$ denote the end state obtained by executing actions $\tau \in \mathbb{R}^{T \times M}$. %of the system after executing the actions $\tau$. 
Let $N_\varepsilon(\alpha) = \{\alpha': ||\alpha' - \alpha||_2 < \varepsilon\}$ be the Euclidean $\varepsilon$-neighbourhood of a latent action $\alpha$.  Then the composition of the maps $\text{Exe} \circ g: \mathbb{R}^{N_\alpha} \rightarrow \mathbb{R}^{N_s}$ mapping from the action latent space to the end state of the system is considered \textit{locally linear} in the neighbourhood of $\alpha$ if there exists an affine transformation 
\begin{align}
f_\alpha:  N_\varepsilon(\alpha) \subset \mathbb{R}^{N_\alpha} \label{eq:aff_trans} &\longrightarrow \mathbb{R}^{N_s} \\ \alpha' &\longmapsto A\alpha' + b \nonumber
\end{align}
such that $\text{Exe}(g(\alpha')) = f_\alpha(\alpha')$ for every $\alpha' \in N_\varepsilon(\alpha)$. We define the \textit{latent local linearity (L3)} of a generative model $g$ to be the mean square error (MSE) of $f_{\alpha_i}$ obtained on $N_\varepsilon(\alpha_i)$ calculated on a subset of latent actions $\{\alpha_i\}$.  %We measure the local linearity of a generative model $g$ on a subset of latent actions $\{\alpha_i\}$ by calculating the mean square error (MSE) of $f_{\alpha_i}$ obtained on $N_\varepsilon(\alpha_i)$. %coefficient of determination $R^2$ of the prediction using $f_\alpha$ as well as 

\subsubsection{Precision and recall} \label{sec:prec_and_recall}
Precision and recall for distributions is a measure, first introduced by \cite{sajjadi2018assessing} and further improved by \cite{kynkaanniemi2019improved}, for evaluating the quality of a distribution learned by a generative model $g$. It is based on the comparison of samples obtained from $g$ with the samples from the ground truth reference distribution. In our case, the reference distribution is the one of the training motor trajectories. Intuitively, \textit{precision} measures the quality of the generated sequences of motor actions by quantifying how similar they are to the training trajectories. It determines the fraction of the generated samples that are realistic. On the other hand, \textit{recall} evaluates how well the learned distribution covers the reference distribution and it determines the fraction of the training trajectories that can be generated by the generative model. In the context of the policy training, we would like the output of $\pi_\Theta$ to be as similar as possible to the demonstrated motor trajectories. It is also important that $\pi_\Theta$ covers the entire state space as it must be able to reach different goal states from different task configurations. Therefore, the generative model needs to have both high precision and high recall scores. 

The improved measure introduced by \cite{kynkaanniemi2019improved} is based on an approximation of
manifolds of both training and generated data. In particular, given a set $\boldsymbol{T} \in \{\boldsymbol{T_r}, \boldsymbol{T_g}\}$ of either real training trajectories $\boldsymbol{T_r}$ or generated trajectories $\boldsymbol{T_g}$, the corresponding manifold is estimated by forming hyperspheres around each trajectory $\tau \in \boldsymbol{T}$ with radius equal to its $k$th nearest neighbour $\NN_k(\tau, \boldsymbol{T})$. To determine whether or not a given novel trajectory $\tau'$ lies within the volume of the approximated manifold we define a binary function
\[
 f(\tau', \boldsymbol{T}) =
  \begin{cases}
  1 & \text{if $||\tau' - \tau||_2 \le ||\tau - \NN_k(\tau, \boldsymbol{T})||_2$ for at least one $\tau \in \boldsymbol{T}$} \\
  0 & \text{otherwise.} 
  \end{cases}
\]
By counting the number of generated trajectories $\tau_g \in \boldsymbol{T}_g$ that lie on the manifold of the real data $\boldsymbol{T}_r$ we obtain the \textit{precision}, and similarly the \textit{recall} by counting the number of real trajectories $\tau_r \in \boldsymbol{T}_r$ that lie on the manifold of the generated data $\boldsymbol{T}_g$
\begin{align*}
    \text{precision}(\boldsymbol{T}_r, \boldsymbol{T}_g) = \frac{1}{|\boldsymbol{T}_g|} \sum_{\tau_g \in \boldsymbol{T}_g} f(\tau_g, \boldsymbol{T}_r) \quad \text{and} \quad
    \text{recall}(\boldsymbol{T}_r, \boldsymbol{T}_g) = \frac{1}{|\boldsymbol{T}_r|} \sum_{\tau_r \in \boldsymbol{T}_r} f(\tau_r, \boldsymbol{T}_g).
\end{align*}
In our experiments, we use the original implementation provided by \cite{kynkaanniemi2019improved} directly on the trajectories as opposed to their representations as suggested in the paper.


==> original/inputs/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Reinforcement learning (RL) can leverage modeling capability of generative models to solve complex sequential decision making problems more efficiently \cite{ghadirzadeh2017deep, arndt2019meta}. 
%Reinforcement learning (RL) combined with generative models is a powerful data-driven approach to solve complex sequential decision-making problems in a data-efficient manner. %that are represented by high-dimensional temporal data with complex dependencies. 
%Reinforcement learning (RL) is a powerful data-driven methodology to solve sequential decision-making problems, and generative models are great tools to model complex dependencies within high-dimensional temporal data in an unsupervised manner. 
%in which a sequence of action-decisions has to be found to complete a given task. 
RL has been applied to end-to-end training of deep visuomotor robotic policies \cite{levine2016end,levine2018learning}
%by maximizing the sum of a reward signal received typically after the execution of every action in the sequence. 
but it is typically too data-inefficient 
%to be applicable to real robotic problems 
especially when applied to tasks that provide only a terminal reward at the end of an episode. %, but not after every time-step that the agent makes an action-decision.
One way to alleviate the data-inefficiency problem in RL is by leveraging prior knowledge to reduce the complexity of the optimization problem.
One prior that significantly reduces the data requirement is an approximation of the distribution from which valid action sequences can be sampled.
Such distributions can be efficiently approximated by training generative models given a sufficient amount of valid action sequences. 
%Generative models hold the promise of modeling complex dependencies within the data, such as motion trajectory of a robotic arm, by learning the approximated distribution in an unsupervised manner.% unsupervised training of the approximated distribution.% from which valid data samples can be drawn. 

The question is then how to combine powerful RL optimization algorithms with the modeling capability of generative models to improve the efficiency of the policy training?
%In other words, how can we leverage the RL optimization power to regulate the generative process to generate proper outputs through an iterative policy training procedure? 
Moreover, which characteristics of the generative models are important for efficient policy training? A suitable generative model must capture the entire distribution of the training data to generate as many distinct motion trajectories as possible, while avoiding the generation of invalid trajectories outside the training dataset. 
The diversity of the generated data enables the policy to complete a given task for the entire set of goal states when training a goal-conditioned policy. On the other hand, adhering to the distribution of the training data ensures safety in generated trajectories which are running on a real robotic platform. 
%Furthermore, from the point of RL optimization, disentangled latent representations of actions are preferred. In a disentangled representation a separate set of dimensions is allocated to control different aspects of the task which leads to a more efficient neural network policy training.


%In this paper, we (i) propose an RL framework combined with a generative model for which we demonstrate it considerably improves the data-efficiency of deep visuomotor policy training to control a robotic arm given raw image pixels as the input, and (ii) show that our proposed measures can be used to evaluate the appropriateness of different latent-variable generative models, thus they can be used to design a guideline to train proper generative models that improve the data-efficiency of the policy training task prior to actual training on a physical robot. 


In this paper, we (i) propose a learning framework that exploits RL and generative models to solve sequential decision making problems and considerably improves the data-efficiency of deep visuomotor policy training to control a robotic arm given raw image pixels as the input,
and (ii) provide a set of measures to evaluate the quality of the latent space of different generative models regulated by the RL policy search algorithms, and use them as a guideline for training the generative models such that the data-efficiency of the policy training can be further improved prior to actual training on a physical robot. 

Regarding (i), the proposed learning framework divides the deep visuomotor sequential decision-making problem into the following sub-problems that can be solved more efficiently:
(a) an unsupervised generative model training problem that approximates the distribution of motor actions, (b) a trust-region policy optimization problem that solves a contextual multi-armed bandit without temporal credit assignment issue which exists in typical sequential decision-making problems, and (c) a supervised learning problem in which we train the deep visuomotor policy in an end-to-end fashion.

%we provide an extensive evaluation of the quality of generative models when combined with the RL policy search algorithm. In particular,
%we study two prominent latent-variable generative models, namely variational auto-encoders (VAEs) \cite{kingma2013auto, higgins2017beta} and generative adversarial networks (GANs) \cite{chen2016infogan}
Regarding (ii), we evaluate generative models based on (a) the quality and coverage of the samples they generate using the precision and recall metric \cite{kynkaanniemi2019improved}, and (b) the quality of their latent representations using two novel measures called \textit{disentangling precision and recall (DPR)} and \textit{latent local linearity (L3)}. Both these measures leverage the end states obtained after execution of the generated trajectories on a robotic platform. Disentanglement measures to which extent individual dimensions in the latent space control different aspects of the task, while local linearity measures the complexity of the generative process and system dynamics in the neighbourhood of each point in the latent space. Our hypothesis is that a generative model that is well disentangled, locally linear and able to generate realistic samples that closely follow the training data (i.e. has high precision and high recall) leads to a more sample efficient %(less samples, higher rewards) 
neural network policy training. We experimentally investigate this hypothesis on several generative models, namely $\beta$-VAEs \cite{higgins2017beta} and InfoGANs \cite{chen2016infogan}, by calculating Pearson's R as well as automatic relevance determination regression (ARD) to quantify the importance of (a) and (b) for a superior RL policy training performance. This evaluation provides a guideline for training latent-variable generative models in a way that enables data-efficient policy training. 


%In particular, we evaluate (a) the quality and coverage of the generated samples using the precision and recall metric \cite{kynkaanniemi2019improved, sajjadi2018assessing}, (b) disentanglement of latent representations using our novel disentanglement metric, (c) the complexity of the generative process using our novel measure of local linearity. Both of our measures (b) and (c) leverage the end states obtained after the execution of the generated trajectories on a robotic platform.


%we provide an extensive evaluation of the quality of generative models when combined with the RL policy search algorithm based on our two novel measures as well as the existing measures for assessing generative models. 

% to better understand the latent structure of different models when regulated by the RL policy search algorithms.
%The generative models are used in our case to generate robot motion trajectories.
%A suitable generative model must capture the widest distribution of the training data to generate as many distinct motion trajectories as possible while avoiding the generation of invalid trajectories outside the training dataset. 
%The diversity of the generated data enables the policy to complete a given task for a wider set of target states. On the other hand, adhering to the distribution of the training data ensures safety in generating trajectories which are running on a real-robotic platform. 
%Furthermore, from the point of RL optimization, disentangled latent representations of actions are preferred. In a disentangled representation a separate set of dimensions is allocated to control different aspects of the task which leads to a more efficient neural network policy training.
%A neural network policy can be trained more efficiently to regulate the generative process in which a disentangled representation is learned such that   a separate set of dimensions is allocated to control different aspects of the task. 
%For example, in a disentangled action representation for a hitting task with a hockey stick, one dimension of the latent variable can be assigned to control the hitting velocity and another dimension for the hitting angel \cite{arndt2019meta}.  

%The main contributions of our work are: 
%(1) introducing a policy optimization method based on expectation-maximization (EM) algorithm that divides a complex visuomotor policy training problem into the three aforementioned downstream tasks that can be solved more efficiently, (2) deriving a new measure for assessing disentanglement of latent representations,
%(3) combining it with three other measures CITE to assess the quality of generative models for efficient policy training, 
%and (4) experimentally studying the characteristics of generative models, more specifically $\beta$-VAEs \cite{higgins2017beta} and InfoGANs \cite{chen2016infogan}, that affect the policy training performance. 
%This paper also provides a comprehensive overview of our earlier work for RL policy training based on generative models \cite{ghadirzadeh2017deep, arndt2019meta, chen2019adversarial,hamalainen2019affordance, butepage2019imitating}

In summary, the advantages of the proposed framework are: 
\begin{itemize}
    \item It improves data-efficiency of the policy training algorithm by at least an order of magnitude by incorporating prior knowledge in terms of a distribution over valid sequences of actions, therefore, reducing the search space. 
    \item It helps to acquire complex visuomotor policies given sparse terminal rewards provided at the end of successful episodes. The proposed formulation converts the sequential decision-making problem into a contextual multi-armed bandit. Therefore, it alleviates the temporal credit assignment problem that is inherent in  sequential decision-making tasks and enables efficient policy training with only terminal rewards.  
    \item It enables safe exploration in RL by sampling actions only from the approximated distribution. 
    This is in stark contrast to the typical RL algorithms in which random actions are taken during the exploration phase. 
    
    \item It provides a set of measures for evaluation of the generative model based on which it is possible to predict the performance of the RL policy training prior to the actual training.
\end{itemize}

This paper provides a comprehensive overview of our earlier work for RL policy training based on generative models \cite{ghadirzadeh2017deep, arndt2019meta, chen2019adversarial,hamalainen2019affordance, butepage2019imitating} and is organized as follows: in Section \ref{sec:related_work}, we provide an overview of the related work. We formally introduce the problem of policy training with generative models in Section \ref{sec:preliminaries}, and describe how the framework is trained in Section \ref{sec:em_policy_training}. In Section \ref{sec:generative_model_training} we first briefly overview VAEs and GANs, and then define all of the evaluation measures used to predict the final policy training performance.  
We present the experimental results in Section \ref{sec:experiments} and discuss the conclusion and future work in Section~\ref{sec:conclusion}.
Moreover, for the sake of completeness, we describe the end-to-end training of the perception and control modules in Appendix \ref{sec:perception} by giving a summary of the prior work \cite{levine2016end, chen2019adversarial}. Note that this work provides a complete overview of the proposed framework and focuses on the evaluation of the generative model. We refer the reader to \cite{ghadirzadeh2017deep} for investigation of the data-efficiency of the proposed approach in training complex visuomotor skills.
%Our code will be made publicly available upon acceptance.




==> original/inputs/perception.tex <==
\section{End-to-end Training of Perception and Control}
\label{sec:perception}
The EM policy training algorithm presented in Section~\ref{sec:em_policy_training} updates the deep policy using the supervised learning objective function introduced in~\eqref{eq:M_loss} (the M-step objective). 
Similar to GPS \cite{levine2016end}, the EM policy training formulation enables simultaneous training of the perception and control parts of the deep policy in an end-to-end fashion. 
In this section, we describe two techniques that can improve the efficiency of the end-to-end training.

\textbf{Input remapping trick}
The input remapping trick \cite{levine2016end} can be applied to condition the variational policy $q$ on a low-dimensional compact state representation, $z$, instead of the high-dimensional states $s$ given by the sensory observations, e.g., camera images. 
The policy training phase can be done in a controlled environment such that extra measures other than the sensory observation of the system can be provided. These extra measures can be for example the position of a target object on a tabletop. 
Therefore, the image observations $s$ can be paired with a compact task-specific state representation $z$ such that $z$ is used in the E-step for updating the variational policy $q_\phi(\alpha|z)$, and $s$ in the M-step for updating the policy $\pi_\theta(\alpha|s)$. 

\textbf{Domain adaptation for perception training}
%The unlabeled images, captured without involving the robot, can be used to improve the data-efficiency of the visuomotor policy training. 
Domain adaptation techniques, e.g., adversarial methods \cite{chen2019adversarial}, can improve the end-to-end training of visuomotor policies with limited robot data samples. 
The unlabeled task-specific images, captured without involving the robot, can be exploited in the M-step to improve the generality of the visuomotor policy to manipulate novel task objects in cluttered backgrounds. 

The M-step is updated to include an extra loss function to adapt data from the two different domains: (i) unlabeled images and (ii) robot visuomotor data. 
The images must contain only one task object in a cluttered background, possibly different than the task object used by the robot during the policy training. 
Given images from the two domains, the basic idea is to extract visual features such that it is not possible to detect the source of the features. 
More details of the method can be found in our recent work in \cite{chen2019adversarial}. 


==> original/inputs/policy_training.tex <==
\section{Expectation-Maximization Policy Training}
\label{sec:em_policy_training}
The EM algorithm is a well-suited approach to find the maximum likelihood solution to the intractable marginalization over the latent variable introduced in~\eqref{eq:margin_tau} and~\eqref{eq:margin_alpha}. 
We use the EM algorithm to find an optimal policy $\pi_{\theta^*}(\alpha|s)$ by first introducing a variational policy $q(\alpha|s)$ which is a simpler auxiliary distribution used to improve the training of $\pi_{\theta}$. 
% which, similar to the policy $\pi_\theta(\alpha|s)$, assigns probability distribution over the latent action variable conditioned on a state.
As the goal is to find an action trajectory $\tau$ that maximizes the reward probability $p(r|s,\tau)$, we start by expressing its logarithm as $\log p(r | s) = \int q(\alpha|s) \log p(r|s) d\alpha$, where we used the identity $\int q(\alpha|s) d\alpha = 1$ and omitted the conditioning on $\tau$ in the reward probability for simplicity.
Following the EM derivation introduced in \cite{neumann2011variational} and using the identity $p(r|s) = p(r,\alpha|s)/p(\alpha |r,s)$, the expression can be further decomposed into
\begin{align}
\log p(r|s) & = \underbrace{\int q(\alpha|s) \log \frac{p(r, \alpha|s)}{q(\alpha|s)} d\alpha}_{\text{I}}  + \underbrace{\int q(\alpha|s) \log \frac{q(\alpha|s)}{p (\alpha | r, s)}\,d\alpha}_{\text{II}} \label{eq:marginal_decomposed} %\\
%& \geq \int q(\alpha|s) \log \frac{p(r, \alpha|s)}{q(\alpha|s)} d\alpha. \nonumber
\end{align}

The second term (II) is the Kullback-Leibler (KL) divergence $D_{KL}( q(\alpha|s) \,||\, p(\alpha |
r,s) )$ between distributions $q(\alpha|s)$ and $p(\alpha |
 r,s)$, which is a non-negative quantity.
Therefore, the first term (I) provides a lower-bound for $\log p(r|s)$. To maximize the latter we use the EM algorithm which is an iterative procedure consisting of two steps known as the expectation (E-) and the maximization (M-) steps, introduced in the following sections. %that instead maximizes the lower-bound in two steps, known as the expectation (E-) and the maximization (M-) steps, introduced in the following sections. 

\subsection{Expectation step } 
\label{sec:EM}
The E-step yields a trust-region policy optimization objective which solves a contextual multi-armed bandit without temporal complexities. The objective of the E-step is to minimize the KL divergence term (II) in~\eqref{eq:marginal_decomposed} by optimizing $q(\alpha | s)$, which in turn indirectly maximizes the lower bound (I).
%is to maximize $\log p(r|s)$ by minimizing the KL divergence term (II) in~\eqref{eq:marginal_decomposed}. 
Since $\log p(r|s)$ does not depend on $q(\alpha|s)$ the sum of the KL divergence term (II) and the lower bound term (I) is a constant value for different $q$. Therefore, reducing (II) by optimizing $q$ increases the lower bound (I). Assuming that $q$ is parametrized by $\phi$, the E-step objective function is given by
\begin{align}
    \phi^* &=\argmin_{\phi} D_{KL}(\,q_\phi(\alpha|s)\,||\,p(\alpha|r,s)\,) \nonumber \\
     &= \argmax_{\phi} \mathbb{E}_{\alpha' \sim q_\phi(\alpha|s)}[\log p(r|s, \alpha')] -  D_{KL}(\,q_\phi(\alpha|s)\,||\,\pi_\theta(\alpha|s)\,),
    \label{eq:E_loss}
\end{align}
where we used the Bayes rule $p(\alpha|r,s) =  p(r|\alpha,s) p(\alpha|s)/p(r|s)$ and substituted $p(\alpha|s)$ by $\pi_\theta (\alpha|s)$. 
%$p(r|\alpha, s)$ is the probability of receiving rewards greater than a threshold value.
In typical RL applications, we maximize the reward value given by a stochastic reward function $r(s,\tau)$. %instead of the probability of receiving a  that the reward is given by a deterministic reward function $r(s, \tau) = r(s, g(\alpha))$.
In this case, $\mathbb{E}_{q_\phi(\alpha|s)}[\log p(r| s, \alpha)]$ can be maximized indirectly by maximizing the expected reward value $\mathbb{E}_{q_{\phi}(\alpha|s)}[r(s, \alpha)]$ on which we can apply the policy gradient theorem. Note that by $r(s, \alpha)$ we refer to $r(s, g_\vartheta(\alpha))$.
Moreover, $D_{KL}(\,q_\phi(\alpha|s)\,||\,\pi_\theta(\alpha|s)\,)$ acts as a trust region term forcing $q_\phi$ not to deviate too much from the policy distribution $\pi_\theta$. 
Therefore, we can apply policy search algorithms with trust region terms to optimize the objective given in~\eqref{eq:E_loss}. Following the derivations introduced in \cite{schulman2015trust}, we adopt TRPO objective for the E-step optimization
\begin{equation}
    \phi^* = \argmax_{\phi} \mathbb{E}_{s' \sim p(s), \alpha' \sim \pi_\theta(\alpha|s')} \left[\frac{q_\phi(\alpha'|s')}{\pi_\theta(\alpha'|s')}\,A(s', \alpha') - D_{KL}(q_\phi(\alpha|s') \, || \, \pi_\theta(\alpha | s'))\right ], 
    \label{eq:trpo}
\end{equation}
where $A(s', \alpha') = r(s', \alpha') - V_\pi(s')$ is the advantage function, $V_\pi(s') = \mathbb{E}_{ \alpha' \sim \pi_\theta(\alpha|s')} [r(s', \alpha')]$ is the value function and $\phi^*$ denotes the optimal solution for the given iteration. Note that the action latent variable $\alpha$ is always sampled from the policy $\pi_\theta(\alpha|s)$ and not from the variational policy $q_\phi(\alpha|s)$.

%In summary, in the E-step, the variational policies are updated based on the reward seeking and the trust region terms given in Eq.~\ref{eq:E_loss}. All policy gradient algorithms that update a policy given a trust region term, such as TRPO \cite{schulman2015trust} or PPO \cite{schulman2017proximal}, can be applied in the E-step to optimize the variational policy. 
%It is worth emphasizing that during the E-step, the policy $\pi_\theta$ is kept fixed. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%% SECTION
\subsection{Maximization step }
The M-step yields a supervised learning objective using which we train the deep policy in an end-to-end fashion. It directly maximizes the lower bound (I) in~\eqref{eq:marginal_decomposed} by optimizing the policy parameters $\theta$ while holding the variational policy $q_\phi$ constant. Following \cite{deisenroth2013survey} and noting that the dynamics of the system $p(r|\alpha, s)$ are not affected by the choice of the policy parameters $\theta$, we maximize (I) by minimizing the following KL divergence
\begin{equation}
\theta^* = \argmin_{\theta} D_{KL}(\,q_\phi(\alpha|s)\, || \,\pi_{\theta}(\alpha|s)\,).
\label{eq:M_loss}
\end{equation}

In other words, the M-step updates the policy $\pi_{\theta}$ to match the distribution of the variational policy $q_\phi$ which was updated in the E-step. Similarly as in the E-step, $\theta^*$ denotes the optimal solution for the given iteration. The M-step can be combined with end-to-end training of the perception and control modules. We refer the reader to the Appendix \ref{sec:perception} for the details.

A summary of the EM policy training is given in Algorithm \ref{alg:training}. In each iteration, a set of states $\{s_i\}$ is sampled from the initial state distribution $p(s)$. For each state $s_i$, a latent action sample $\alpha_i$ is sampled from the distribution given by the policy $\pi_\theta(\alpha|s_i)$. A generative model $g$ is then used to map every latent action variable $\alpha_i$ into a full motor trajectory $\tau_i$ which is then deployed on the robot to get the corresponding reward value $r_i$. 
In the inner loop, the variational policy $q_\phi$ and the main policy $\pi_\theta$ are updated iteratively based on gradient descent on batches of data using the objective function for the E- and M-steps of the policy optimization method.
\input{inputs/algorithm}

%\subsection{Multi-agent learning}
%The number of variational policies can be chosen arbitrarily. In the E-step, several variational policies can be simultaneously optimized by splitting the state space into smaller sub spaces for each of which one variational policy is optimized. This can improve the efficiency of the policy training since variational policies with fewer parameters have to be optimized in smaller regions of the state space. The analysis of the effect of the number of the variational policies for the policy training is presented in the experimental result section. 

==> original/inputs/related_work.tex <==
\section{Related work}
\label{sec:related_work}

Our work addresses two types of problems: 
(a) visuomotor policy training based on unsupervised generative model training and trust-region policy optimization, and
(b) evaluation of generative models to forecast the efficiency of the final policy training task. 
We introduce the related work for each of the problems in the following sections. 

\textbf{Data-efficient end-to-end policy training:}
In recent years, end-to-end training of visuomotor policies using deep RL has gained in popularity in robotics research \cite{ghadirzadeh2017deep, levine2016end, finn2016deep, kalashnikov2018qt, quillen2018deep, singh2017gplac, devin2018deep, pinto2017asymmetric}. 
However, deep RL algorithms are typically data-hungry and learning a general policy, i.e., a policy that performs well also for previously unseen inputs, requires a farm of robots continuously collecting data for several days \cite{levine2018learning, finn2017deep, gu2017deep, dasari2019robonet}.
The limitation of large-scale data collection has hindered the applicability of RL solutions to many practical robotics tasks. Recent studies tried to improve
%tried to address this issue by developing different techniques to improve 
the data-efficiency by training the policy in simulation and transferring the acquired visuomotor skills to the real setup \cite{quillen2018deep, pinto2017asymmetric, abdolmaleki2020distributional, peng2018sim}, a paradigm known as sim-to-real transfer learning. 
%Policy training in simulation and transferring the acquired visuomotor skills to the real setup, a paradigm known as sim-to-real transfer learning, is a typical solution to provide more data to the learning agent to improve the efficiency of the policy training \cite{quillen2018deep, pinto2017asymmetric, abdolmaleki2020distributional, peng2018sim}.
Sim-to-real approaches are utilized for two tasks in deep policy training: (i) training the perception model via randomization of the texture and shape of visual objects in simulation and using the trained model directly in the real world setup (zero-shot transfer) \cite{hamalainen2019affordance, tobin2017domain}, and (ii) training the policy in simulation by randomizing the dynamics of the task and transferring the policy to the real setup by fine-tuning it with the real data (few-shot transfer learning) \cite{arndt2019meta, peng2018sim}. 
However, challenges in the design of the simulation environment can cause large differences between the real and the simulated environments which hinder an efficient knowledge transfer between these two domains. 
In such cases, transfer learning from other domains, e.g., human demonstrations \cite{butepage2019imitating, yu2018one} or simpler task setups \cite{chen2019adversarial, chen2018deep}, can help the agent to learn a policy more efficiently. 
In this work, we exploit human demonstrations to shape the robot motion trajectories by training generative models that reproduce the demonstrated trajectories. 
Following our earlier work \cite{chen2019adversarial}, we exploit adversarial domain adaptation techniques \cite{tzeng2017adversarial, tzeng2020adapting} to improve the generality of the acquired policy when it is trained in a simple task environment with a small amount of training data. 
In the rest of this section, we review related studies that improve the data-efficiency and generality of RL algorithms by utilizing trust-region terms, converting the RL problem into a supervised learning problem, and trajectory-centered approaches that shape motion trajectories prior to the policy training.

Improving the policy while avoiding abrupt changes in the policy distribution after each update is known as the trust-region approach in policy optimization. 
Trust-region policy optimization (TRPO) \cite{schulman2015trust} and proximal policy optimization (PPO) \cite{schulman2017proximal} are two variants of trust-region policy gradient methods that scale well to non-linear policies such as neural networks.
%Schulman et al. introduced two policy gradient methods, trust-region policy optimization (TRPO) \cite{schulman2015trust} and proximal policy optimization (PPO) \cite{schulman2017proximal}, that scale well to non-linear policies such as neural networks.
The key component of TRPO and PPO is a surrogate objective function with a trust-region term based on which the policy can be updated and monotonically improved. % while the policy distribution is not abruptly changed after each iteration. 
In TRPO, the changes in the distributions of the policies before and after each update are penalized by a KL divergence term. 
Therefore, the policy is forced to stay in a trust-region given by the action distribution of the current policy. 
Our EM formulation yields a similar trust-region term with the difference being that it penalizes the changes in the distribution of the deep policy and a so-called variational policy that will be introduced as a part of our proposed optimization algorithm. Since our formulation allows the use of any policy gradient solution, we use the same RL objective function as in TRPO. 

The EM algorithm has been used for policy training in a number of prior work \cite{neumann2011variational ,deisenroth2013survey,levine2013variational}. The key idea is to introduce variational policies to decompose the policy training into two downstream tasks that are trained iteratively until no further policy improvement can be observed \cite{ghadirzadeh2018sensorimotor}. 
In \cite{levine2016end} the authors introduced the guided policy search (GPS) algorithm which divides the visuomotor policy training task into a trajectory optimization and a supervised learning problem. 
GPS alternates between two steps: (i) optimizing a set of trajectories by exploiting a trust-region term to stay close to the action distribution given by the deep policy, and (ii) updating the deep policy to reproduce the motion trajectories. 
Our EM solution differs from the GPS framework and earlier approaches in that we optimize the trajectories by regulating a generative model that is trained prior to the policy training. 
Training generative models enables the learning framework to exploit human expert knowledge as well as to optimize the policy given only terminal rewards as explained earlier.

Trajectory-centric approaches, such as dynamic movement primitives (DMPs), have been popular because of the ease of integrating expert knowledge in the policy training process via physical demonstration \cite{peters2006policy, peters2008reinforcement, ijspeert2003learning, ijspeert2013dynamical, hazara2019transferring}.
However, such models are less expressive compared to deep neural networks and are particularly limited when it comes to end-to-end training of the perception and control elements of the model. Moreover, these approaches cannot be used to train reactive policies where the action is adjusted in every time-step based on the observed sensory input \cite{haarnoja2018composable}. 
On the other hand, deep generative models can model complex dependencies within the data by learning the underlying data distribution from which realistic samples can be obtained. 
Furthermore, they can be easily accommodated in larger neural networks without affecting the data integrity. Our framework based on generative models enables training both feedback (reactive) and feedforward policies by adjusting the policy network architecture. 

The use of generative models in robot learning has become popular in recent years \cite{ghadirzadeh2017deep, butepage2019imitating, hamalainen2019affordance, chen2019adversarial, arndt2019meta, lippi2020latent, gothoskar2020learning, igl2018deep, buesing2018learning, mishra2017prediction, ke2018modeling, hafner2018learning, rhinehart2018deep, krupnik2019multi} because of their  low-dimensional and regularized latent spaces. % that are typically obtained by training generative models. 
However, latent variable generative models are mainly studied to train a long-term state prediction model that is used in the context of trajectory optimization and model-based reinforcement learning  \cite{buesing2018learning, mishra2017prediction, ke2018modeling, hafner2018learning, rhinehart2018deep, krupnik2019multi}.
Regulating generative models based on reinforcement learning to produce sequences of actions according to the  visual state has first appeared in our prior work \cite{ghadirzadeh2017deep}. Since then we applied the framework in different robotic tasks, e.g., throwing balls \cite{ghadirzadeh2017deep}, shooting hockey-pucks \cite{arndt2019meta}, pouring into mugs \cite{chen2019adversarial, hamalainen2019affordance}, and in a variety of problem domains, e.g., sim-to-real transfer learning \cite{hamalainen2019affordance, arndt2019meta} and domain adaptation to acquire general policies \cite{chen2019adversarial}. 
%This work is a comprehensive study that builds the theoretical foundation of our earlier work and in addition studies the characteristics of the generative models that can affect the efficiency of the policy training task.  

\textbf{Evaluation of generative models:}
Although generative models have proved successful in many domains \cite{lippi2020latent, brock2018large, wang2018high, vae_anom, vae_text8672806} assessing their quality remains a challenging problem \cite{challenging_common}. It involves analysing the quality of both latent representations and generated samples. %A general belief is that a superior model possesses a well structured latent space and tightly matches the distribution of the training data. %The evaluation is commonly studied on models trained on image data for which we have a good understanding and are therefore able to explain the empirical findings in a more intuitive way. 
Regarding the latter, generated samples and their variation should resemble those obtained from the training data distribution. Early developed metrics such as IS \cite{IS_NIPS2016_6125}, FID \cite{FID_NIPS2017_7240} and KID \cite{binkowski2018demystifying} provided a promising start but were shown to be unable to separate between failure cases, such as mode collapse or unrealistic generated samples \cite{sajjadi2018assessing, kynkaanniemi2019improved}. Instead of using a one-dimensional score, \cite{sajjadi2018assessing} proposed to evaluate the learned distribution by comparing the samples from it with the ground truth training samples using the notion of precision and recall. Intuitively, precision measures the similarity between the generated and real samples, while recall determines the fraction of the true distribution that is covered by the distribution learned by the model. The measure was further improved both theoretically and practically by \cite{revisiting_pr}, while \cite{kynkaanniemi2019improved} provides an explicit non-parametric variant of the original probabilistic approach. We complement our measures for assessing disentanglement and local linearity of the latent representations with the precision and recall measure provided by \cite{kynkaanniemi2019improved}.


Regarding the assessment of the quality of the latent representation,
a widely adopted approach 
%for assessing the quality of the latent representations 
is the measure of disentanglement \cite{higgins2018towards, repr_learning_survey, tschannen2018recent}. A representation is said to be disentangled if each latent component encodes exactly one ground truth generative factor present in the data \cite{kim2018disentangling}. Existing frameworks for both learning and evaluating disentangled representations \cite{higgins2017beta, kim2018disentangling, eastwood2018framework, chen2018isolating,kumar2017variational} rely on the assumption that the ground truth factors of variation are known a priori and are independent. The core idea is to measure how changes in the generative factors affect the latent representations and vice versa. In cases when an encoder network is available, this is typically achieved with a classifier that was trained to predict which generative factor was held constant given a latent representation \cite{higgins2017beta, kim2018disentangling, eastwood2018framework, kumar2017variational, chen2018isolating}. In generative models without an encoder network, such as GANs, disentanglement is measured by visually inspecting the latent traversals provided that the input data are images \cite{chen2016infogan, jeon2019ibgan, lee2020high, liu2019oogan}. However, these measures are difficult to apply when generative factors of variation are unknown or when manual visual inspection is not possible,
%when the ground truth factors of variation are unknown or input data are not images, 
both of which is the case with sequences of motor commands for controlling a robotic arm. We therefore define a measure of disentanglement that does not rely on any of these requirements and instead
%does not rely on any prior knowledge of generative factors nor on manual visual inspection of generated samples. Instead, it 
leverages the end states of the downstream robotics task corresponding to a given set of latent action representations. In contrast to existing measures it measures how changes in the latent space affect the obtained end states in a fully unsupervised way. Moreover, since the generative model in our case is combined with the system dynamics, we complement the evaluation of the latent representations with a measure of local linearity which quantifies the complexity of the system dynamics in a neighbourhood of a given latent sample.

%Assessing the quality of the learned distribution and samples from it presents a separate challenge.





==> original/inputs/reserved.tex <==
\begin{figure}
\centering
\begin{minipage}{.4\textwidth}
  \centering
  \includegraphics[height=.7\linewidth]{figures/MMDalpha10_basecolorsGroup11_disentanglement_scores_dict_1589354519359854.png}
  \captionof{figure}{Policy training}
  \label{fig:test1}
\end{minipage}%
\hspace{0cm}
\begin{minipage}{.4\textwidth}
  \centering
  \includegraphics[height=0.7\linewidth]{figures/MMDalpha10_basecolorsGroup21_disentanglement_scores_dict_1589354519359854.png}
  \captionof{figure}{Disentanglement score}
  \label{fig:test2}
\end{minipage}
\end{figure}

==> original/inputs/todo.tex <==
\section{TODO list}
\paragraph{Final comments}
\begin{itemize}

\item Eq, Sec, Fig vs Equation, Section, Figure
%\item : vs , before align environment
\item action latent variable vs latent action variable
\item KL, DKL, KL-divergence?
\item Explicit naming of authors in the first part of the related work, why?
\item When we have expected values it is not mathematically correct to write neither $\mathbb{E}_{\alpha ~p(.)}[x]$ (not clear what is the dot) nor $\mathbb{E}_{\alpha ~p(alpha)}[x]$ (the left hand side $\alpha$ is a concrete sample while the right hand side one is a function variable). I would therefore suggest to kill the explicit sampling from the notation and always write $\mathbb{E}_{p(\alpha)}[x]$. It is a standard way to denote expectations in the statistics i believe.
\item In section GANs, we say that we use InfoGAN because it encouranges the disentanglement. However, we do not mention it in VAEs even though we do use a higher $\beta$ which encouranges disentanglement. I think we should have a sentence about it there as well. 
\item It seems like I trained GANs for 1000 epochs while you trained VAEs for 10000. This causes some implicit differences in the evaluation metrics (like VAEs are always better), shall we say something about it? 
\item Read through the appendix
\begin{comment}

\item Decide on the disentanglement metric. Read the following papers (links included):        
    \begin{itemize}
    \item \href{https://openreview.net/pdf?id=Sy2fzU9gl}{BetaVAE metric} cited in \href{https://arxiv.org/pdf/1903.11260.pdf}{Small Data Challenges in Big Data Era}, section Disentanglement Metric page 8
    \item \href{https://arxiv.org/pdf/1905.13662.pdf}{On the fairness of disentangled representations} - The authors said at NeurIPS that the most reliable metric is DCI
    \item Potentially also \href{https://arxiv.org/pdf/1905.12506.pdf}{Are Disentangled Representations Helpful for Abstract Visual Reasoning?} - on their poster it looked like they compared many different ones using VAEs, might be relevant
    \end{itemize}

\item Decide on IS and FID score, do we want to implement both? Read the following papers (links included):
    \begin{itemize}
        \item \href{https://arxiv.org/pdf/1901.01091.pdf}{Adaptive Density Estimation for GMs} - see Table 3 for different score benchmarks. The IS and FID metrics are explained and referenced in Appendix D. Also, the authors claimed at their poster that they learned disentangled representations but they didn't do any study on that in the paper.
    \end{itemize}
\end{comment}
    

\end{itemize}
\begin{comment}
\Large{
$\textbf{g}$
\\
${\color{orange}\{\tau = g(\alpha) \,|\, \alpha_l = I_d \}}$ \\
${\color{teal}\{\tau\,|\,\tau \sim p(\tau) \}}$
\\
$\textbf{Env}$
\\
${\color{orange}\boldsymbol{S}_g^{l-Id} = \{s_g^1, \dots, s_g^n\}}$ \\
${\color{teal}\boldsymbol{S}_r = \{s_r^1, \dots, s_r^n\}}$
\\
$\boldsymbol \proj_j$
\\
${\color{orange}\proj_j \boldsymbol{S}_g^{l-Id} = \{\proj_j s_g^1, \dots, \proj_j s_g^n\}}$ \\
${\color{teal}\proj_j \boldsymbol{S}_r = \{\proj_j s_r^1, \dots, \proj_j s_r^n\}}$

$\MMD(\proj_j \boldsymbol{S}_g^{l-Id}, \proj_j \boldsymbol{S}_r)$
\\
{\color{gray} phase 1} \\
{\color{gray} phase 2}}
\end{comment}
